Prevalence of Earth-size planets orbiting Sun-like stars

Determining whether Earth-like planets are common or rare looms as a touchstone in the question of life in the universe. We searched for Earth-size planets that cross in front of their host stars by examining the brightness measurements of 42,000 stars from National Aeronautics and Space Administration's Kepler mission. We found 603 planets, including 10 that are Earth size (1-2 Earth-radii) and receive comparable levels of stellar energy to that of Earth (within a factor of four). We account for Kepler's imperfect detectability of such planets by injecting synthetic planet-caused dimmings into the Kepler brightness measurements and recording the fraction detected. We find that $11\pm4%$ of Sun-like stars harbor an Earth-size planet receiving between one and four times the stellar intensity as Earth. We also find that the occurrence of Earth-size planets is constant with increasing orbital period (P), within equal intervals of logP up to $\sim200$ d. Extrapolating, one finds $5.7^{+1.7}_{-2.2}%$ of Sun-like stars harbor an Earth-size planet with orbital periods of 200-400 d.

==> replacebib <==
#!/bin/tcsh -f
#(ie run the tshell on this but don't read the .cshrc or .tcshrc)

set ver = "version = 1.05 of replacebib 2012 Jun 19"
#       2012 Jun 19, 1.05: upgrade according to Ren?e Otte's email
#       2012 Jun 19, 1.03: merge two versions of replacebib!
#                          comment out original bibliography call!
#       2009 Nov 14, 1.02: improve version description
#       2009 Jun 26, 1.01: functional - add author documentation
#       2009 Jun 26, 1.00: origin 

if ($#argv == 0) then
   echo 'usage: replacebib [source name] [target name]'
   echo 'Replace the bibliography calls in a LaTeX document'
   echo 'with the bibliography text itself.' # usage
   echo 'This is required by PNAS as described in the instructions at' # usage
   echo 'http://www.pnas.org/site/misc/LaTex.shtml' # usage

   echo
   echo 'The source is the latex file to use as input.'
   echo 'The target is the latex file with the bibliography inserted.'

   echo
   echo 'SET UP:'

   echo
   echo '1. Below your \begin{document} line put this line:'
   echo '\bibliographystyle{pnas}'
   echo 'Use the pnas.bst file available from'
   echo 'http://www.ccrnp.ncifcrf.gov/~toms/latex.html'
   echo "(Note: You can use any format, this program won't care.)"

   echo
   echo '2. At the point where your bibliograph should go, insert:'
   echo '\bibliography{all}'
   echo 'where "all" is the name of your bibliograph database eg "all.bib".'
   echo 'This is just above "\end{article}" for the PNAS style.'

   echo
   echo '3. Use the pnas.bst file available from'
   echo 'http://www.ccrnp.ncifcrf.gov/~toms/latex.html'

   echo
   echo '4. Run latex to create your source.bbl file.'

   echo
   echo 'WHAT THIS PROGRAM DOES:'
   echo
   echo 'Remove the \bibliographystyle{pnas} line.'
   echo 'Replace \bibliography{...} with the source bbl file.'

   echo
   echo 'If there is only one argument (any token) then:'
   echo '- the source is set to "paper"'
   echo '- the target is set using the version name.'
   echo 'The version name is on a line containing "version = "'.
   echo 'The version name is a space delimited word containing ".tex".'

   # The version can be found by the ver program:
   # http://alum.mit.edu/www/toms/delila/ver.html
   # However, this is coded into replacebib so there is no dependency.

   echo
   echo 'For example if your paper contains:'
   echo '   \newcommand{\theversion}%'
   echo '      {{version = 1.88 of emmgeo.tex 2009 Nov 10}}'
   echo 'and you run this script with the argument "-bib":'
   echo '     replacebib -bib'
   echo 'then the target name will be "emmgeo-bib.tex"'

   echo
   echo 'RESULTS:'
   echo
   echo 'The output target file is generated.'
   echo 'The program reports the line where the biblography was inserted'
   echo 'and show the first few and last difference lines'
   echo 'between the input and output files.'
   echo 'You should verify that the \bibliographystyle{pnas}'
   echo 'line is gone and that the entire bibliography has been inserted.'

   echo
   echo "Permanent location of this program:"
   echo "http://alum.mit.edu/www/toms/ftp/replacebib"

   echo
   echo "$ver"
   echo

   echo "  Dr. Thomas D. Schneider"
   echo "  National Institutes of Health"
   echo "  schneidt@mail.nih.gov"
   echo "  toms@alum.mit.edu (permanent)"
   echo "  http://alum.mit.edu/www/toms (permanent)"
   exit
endif

if ($#argv == 1) then
   set source = 'paper'
   # now use paper.tex to find the target name

   if !(-f ${source}.tex) then
      echo "There is no ${source}.tex file."
      exit 
   #else
   #   echo "${source}.tex exists."
   endif
   set version = "`grep 'version =' ${source}.tex`"
   if ("$version" == '') then
      echo 'No version line exists - HALT'
      exit
   endif
   echo "Using version line:"
   echo "$version"
   set rawtarget = `echo "$version" | tr ' ' '\n' | grep '.tex' `
   set target = `echo "$rawtarget" | sed "s/.tex/$1/"`
else
   set source = `echo $1 | sed 's/.tex//'`
   set target = `echo $2 | sed 's/.tex//'`
endif

if !(-f ${source}.tex) then
   echo There is no ${source}.tex file.
   exit 
else
   echo "source ${source}.tex exists."
endif

if !(-f ${source}.bbl) then
   echo There is no ${source}.bbl file.
   exit 
else
   echo "source ${source}.bbl exists."
endif

echo the target name is: "${target}.tex"

if ("${target}.tex" == "${source}.tex") then
   echo "${source}.tex = ${target}.tex - HALT to avoid overwriting source"
   exit
endif

# echo ---- thingy
# grep '\\bibliography{' ${source}.tex
# echo ----
# exit

# 2012 Jun 19
# On Sun OS
# grep '\bibliography{' ${source}.tex
# works and identifies the bibliography line.
# On Mac OS X 10.6.8 and Cygwin this
# fails to find the bibliography line.  However
# grep '\\bibliography{' ${source}.tex
# or
# grep 'bibliography{' ${source}.tex
# works on Sun and OS X.  Thanks to R.A. Otte for this tip.

# grep '\bibliography{' ${source}.tex
set breakpoint = `grep -n '\\bibliography{' ${source}.tex|tr ':' '\n' |head -1`
if ("$breakpoint" == '') then
   echo "'\bibliography{' is NOT in ${source}.tex"
   exit
endif
echo "'\bibliography{' is in ${source}.tex at line $breakpoint"
@ headpart = $breakpoint - 1

head -${headpart} ${source}.tex |\
grep -v '\\bibliographystyle{' |\
cat > ${target}.tex

# echo "new stuff" >> ${target}.tex
cat "${source}.bbl" >> ${target}.tex

tail -n +${breakpoint} ${source}.tex |\
sed 's/\\bibliography{/% original source: \\bibliography{/' |\
cat >> ${target}.tex

#cat ${target}.tex

echo "------- diff ${source}.tex ${target}.tex | head"
diff ${source}.tex ${target}.tex | head

echo "------- diff ${source}.tex ${target}.tex | tail"
diff ${source}.tex ${target}.tex | tail
echo "-------"



==> tab1.tex <==
  1026032 &    8.5 &  133.8 &        NaN &         eclipse &  4.1e-01 &  9.0e-04 &  6044 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   42.1 &  NaN \\
  1026957 &   21.8 &  144.8 &  K00958.01 &          planet &  3.1e-02 &  4.2e-03 &  4861 &     66 &   4.6 &  1.5e-02 &    0.7 &  2.1e-02 &   SM &    2.5 &  0.3 \\
  1571511 &   14.0 &  135.5 &  K00362.01 &         eclipse &  1.3e-01 &  3.2e-05 &  6055 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   14.5 &  NaN \\
  1718189 &   21.9 &  144.3 &  K00993.01 &          planet &  1.7e-02 &  9.8e-04 &  5827 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.7 &  NaN \\
  1849702 &   39.8 &  155.6 &  K02538.01 &          planet &  1.7e-02 &  3.7e-03 &  5023 &     61 &   4.6 &  2.5e-02 &    0.7 &  3.4e-02 &   SM &    1.4 &  0.3 \\
  1872821 &   10.3 &  134.6 &  K02351.01 &          planet &  1.8e-02 &  1.1e-03 &  5706 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.7 &  NaN \\
  2141783 &  116.5 &  144.1 &  K02201.01 &          planet &  2.5e-02 &  3.7e-03 &  6063 &     64 &   4.2 &  1.6e-01 &    1.5 &  3.2e-01 &   SM &    4.1 &  1.1 \\
  2164169 &   32.3 &  133.9 &  K01029.01 &          planet &  2.3e-02 &  7.4e-04 &  5975 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.4 &  NaN \\
  2166206 &    8.1 &  132.7 &  K01028.01 &        vardepth &  1.8e-02 &  8.8e-04 &  6014 &    -99 &   4.2 &      NaN &    1.4 &      NaN &    P &    2.7 &  NaN \\
  2304320 &   16.5 &  133.9 &  K02033.01 &          planet &  1.8e-02 &  8.6e-04 &  5061 &     58 &   4.6 &  3.2e-02 &    0.7 &  3.9e-02 &   SM &    1.4 &  0.1 \\
  2305255 &   24.6 &  156.0 &        NaN &          planet &  2.1e-02 &  5.2e-04 &  5980 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.2 &  NaN \\
  2306740 &   10.3 &  138.7 &        NaN &         eclipse &  5.5e-01 &  1.3e-03 &  5932 &    -99 &   4.2 &      NaN &    1.3 &      NaN &    P &   75.4 &  NaN \\
  2309719 &   54.4 &  164.1 &  K01020.01 &          Vshape &  1.6e-01 &  4.0e-03 &  6159 &     71 &   4.3 &  1.0e-01 &    1.3 &  1.9e-01 &   SM &   23.4 &  3.4 \\
  2438264 &   15.9 &  146.1 &  K00440.01 &          planet &  2.8e-02 &  1.2e-03 &  5070 &     55 &   4.6 &  1.7e-02 &    0.8 &  2.2e-02 &   SM &    2.4 &  0.1 \\
  2441495 &   12.5 &  138.5 &  K00166.01 &          planet &  2.4e-02 &  4.6e-04 &  5208 &     82 &   4.6 &  1.5e-02 &    0.8 &  1.7e-02 &   SM &    2.1 &  0.1 \\
  2444412 &   14.9 &  141.3 &  K00103.01 &          planet &  2.8e-02 &  1.4e-03 &  5554 &     78 &   4.5 &  6.0e-02 &    0.9 &  6.8e-02 &   SM &    2.8 &  0.2 \\
  2449431 &   86.8 &  170.3 &  K02009.01 &          planet &  2.1e-02 &  1.6e-03 &  5578 &    129 &   4.4 &  2.9e-02 &    0.9 &  2.1e-02 &   SM &    2.1 &  0.2 \\
  2557816 &    9.4 &  138.9 &  K00488.01 &          planet &  2.6e-02 &  1.5e-03 &  5770 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.6 &  NaN \\
  2571238 &    9.3 &  136.0 &  K00084.01 &          planet &  2.4e-02 &  2.9e-04 &  5523 &     78 &   4.5 &  4.5e-02 &    0.9 &  4.6e-02 &   SM &    2.3 &  0.1 \\
  2576692 &   87.9 &  194.1 &        NaN &          Vshape &  7.5e-01 &  5.1e-02 &  5801 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   71.1 &  NaN \\
  2580872 &   15.9 &  145.5 &        NaN &         eclipse &  7.2e-01 &  7.0e-03 &  5434 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   68.8 &  NaN \\
  2695110 &   44.2 &  165.8 &  K00400.01 &        vardepth &  9.4e-02 &  8.8e-03 &  6089 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   10.6 &  NaN \\
  2715135 &    5.7 &  133.3 &  K01024.01 &          planet &  2.4e-02 &  1.1e-03 &  4302 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.5 &  NaN \\
  2716979 &    8.8 &  137.7 &        NaN &          planet &  7.9e-03 &  5.5e-04 &  6098 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &    1.0 &  NaN \\
  2837111 &    8.7 &  135.1 &  K01110.01 &          planet &  1.6e-02 &  7.4e-04 &  5948 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.6 &  NaN \\
  2854698 &    8.2 &  138.1 &  K00986.01 &          planet &  2.2e-02 &  1.0e-03 &  5475 &     72 &   4.5 &  2.3e-02 &    0.9 &  3.8e-02 &   SM &    2.1 &  0.1 \\
  2985767 &   14.1 &  140.0 &  K02032.01 &          planet &  1.2e-02 &  6.4e-04 &  5530 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.1 &  NaN \\
  2987027 &   17.3 &  133.8 &  K00197.01 &          planet &  9.2e-02 &  1.0e-03 &  4945 &     40 &   4.6 &  1.3e-02 &    0.7 &  1.8e-02 &   SM &    7.4 &  0.2 \\
  2990873 &   16.2 &  136.0 &  K02335.01 &          planet &  1.5e-02 &  1.2e-03 &  5555 &     83 &   4.5 &  6.1e-02 &    0.9 &  7.4e-02 &   SM &    1.5 &  0.2 \\
  3002478 &    6.4 &  135.5 &  K02380.01 &          planet &  1.5e-02 &  7.7e-04 &  5951 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.5 &  NaN \\
  3003991 &    7.2 &  131.9 &        NaN &         eclipse &  2.8e-01 &  2.2e-03 &  5532 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   24.4 &  NaN \\
  3098194 &   30.5 &  137.0 &        NaN &        vardepth &  7.1e-01 &  1.7e-02 &  5484 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   74.6 &  NaN \\
  3098197 &   30.5 &  137.0 &        NaN &        vardepth &  4.2e-01 &  6.9e-03 &  5962 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   42.1 &  NaN \\
  3102024 &   13.8 &  139.5 &        NaN &         eclipse &  6.7e-01 &  3.6e-03 &  5353 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   56.7 &  NaN \\
  3102384 &   10.6 &  132.8 &  K00273.01 &          planet &  1.6e-02 &  4.0e-04 &  5672 &     80 &   4.4 &  6.4e-02 &    1.1 &  9.1e-02 &   SM &    1.9 &  0.2 \\
  3109930 &   37.8 &  158.4 &  K01112.01 &          planet &  2.0e-02 &  7.6e-04 &  6099 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.2 &  NaN \\
  3116412 &   13.0 &  136.3 &  K01115.01 &          planet &  1.5e-02 &  6.8e-04 &  5760 &     31 &   4.2 &  7.2e-02 &    1.3 &  1.1e-01 &   SM &    2.1 &  0.2 \\
  3120308 &   10.3 &  136.5 &        NaN &  offset-no-star &  1.5e-02 &  1.3e-03 &  5706 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.5 &  NaN \\
  3120320 &   10.3 &  136.5 &        NaN &         eclipse &  4.8e-01 &  2.3e-02 &  5903 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   48.8 &  NaN \\
  3120904 &   42.9 &  139.9 &        NaN &          planet &  1.2e-02 &  8.0e-04 &  6152 &     63 &   4.3 &  1.1e-01 &    1.2 &  1.9e-01 &   SM &    1.6 &  0.3 \\
  3128552 &    8.7 &  133.0 &  K02055.01 &          planet &  2.1e-02 &  9.8e-04 &  5748 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &    2.0 &  NaN \\
  3128793 &   24.7 &  137.8 &  K01786.01 &          planet &  8.3e-02 &  7.5e-04 &  4669 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    5.7 &  NaN \\
  3217264 &   29.2 &  156.2 &  K00401.01 &          planet &  4.1e-02 &  4.7e-04 &  5363 &     43 &   4.5 &  5.2e-03 &    0.9 &  5.2e-03 &   SM &    4.0 &  0.1 \\
  3218908 &   18.9 &  149.5 &  K01108.01 &          planet &  2.4e-02 &  1.3e-03 &  5546 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
  3219037 &   10.0 &  136.8 &        NaN &          planet &  9.9e-03 &  9.4e-04 &  5948 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.0 &  NaN \\
  3223433 &   61.1 &  132.5 &        NaN &          planet &  1.4e-02 &  3.3e-03 &  5518 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.2 &  NaN \\
  3230753 &   17.7 &  143.9 &  K02928.01 &          planet &  1.4e-02 &  8.0e-04 &  5250 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.2 &  NaN \\
  3230787 &   17.7 &  143.9 &        NaN &        vardepth &  5.9e-01 &  1.8e-02 &  5905 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   65.0 &  NaN \\
  3231341 &   12.3 &  137.6 &  K01102.01 &          planet &  2.0e-02 &  1.2e-03 &  6005 &    194 &   4.2 &  1.8e-01 &    1.4 &  3.7e-01 &   SM &    3.1 &  0.8 \\
  3236705 &   83.3 &  194.3 &        NaN &          planet &  2.3e-02 &  3.2e-03 &  5965 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.4 &  NaN \\
  3239671 &  148.0 &  263.1 &  K02066.01 &          planet &  3.4e-02 &  3.3e-03 &  5573 &     45 &   4.4 &  4.3e-02 &    0.9 &  4.1e-02 &   SM &    3.4 &  0.4 \\
  3323289 &   33.7 &  158.9 &        NaN &         eclipse &  6.7e-01 &  2.8e-04 &  5401 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &   65.4 &  NaN \\
  3323887 &   19.3 &  144.0 &  K00377.01 &             ttv &  8.0e-02 &  1.6e-02 &  5780 &     37 &   4.4 &  6.3e-02 &    1.0 &  7.6e-02 &   SM &    9.0 &  1.9 \\
  3326377 &  198.7 &  156.5 &        NaN &          planet &  4.3e-02 &  1.9e-03 &  5180 &     41 &   4.6 &  2.9e-02 &    0.8 &  3.4e-02 &   SM &    3.7 &  0.2 \\
  3337425 &    7.0 &  132.7 &  K01114.01 &          planet &  1.5e-02 &  7.6e-04 &  5721 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.7 &  NaN \\
  3342467 &   88.2 &  209.2 &        NaN &          planet &  3.0e-02 &  2.7e-03 &  5414 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.6 &  NaN \\
  3342592 &   17.2 &  136.2 &  K00402.01 &         eclipse &  1.4e-01 &  5.2e-04 &  6004 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   13.9 &  NaN \\
  3353050 &    5.1 &  133.8 &  K00384.01 &          planet &  1.4e-02 &  4.2e-04 &  6156 &     48 &   4.4 &  3.2e-02 &    1.1 &  5.1e-02 &   SM &    1.7 &  0.1 \\
  3433668 &   15.0 &  143.7 &        NaN &          planet &  9.8e-03 &  9.5e-04 &  5823 &    256 &   4.2 &  1.8e-01 &    1.4 &  4.3e-01 &   SM &    1.5 &  0.5 \\
  3442055 &   29.6 &  133.7 &  K01218.01 &          planet &  1.6e-02 &  5.9e-04 &  5624 &     88 &   4.4 &  5.8e-02 &    1.0 &  7.9e-02 &   SM &    1.8 &  0.2 \\
  3446746 &   13.1 &  135.4 &  K00385.01 &          planet &  1.9e-02 &  1.2e-03 &  5412 &     61 &   4.5 &  5.0e-02 &    0.9 &  4.8e-02 &   SM &    1.9 &  0.2 \\
  3448130 &   78.5 &  144.1 &  K02043.01 &  offset-no-star &  2.2e-02 &  1.6e-03 &  6005 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.3 &  NaN \\
  3531558 &   25.0 &  138.7 &  K00118.01 &          planet &  1.5e-02 &  7.0e-04 &  5807 &     59 &   4.3 &  6.0e-02 &    1.1 &  8.5e-02 &   SM &    1.8 &  0.2 \\
  3534118 &  178.4 &  218.2 &        NaN &          Vshape &  2.0e-01 &  3.1e-02 &  6079 &    139 &   4.3 &  2.4e-02 &    1.1 &  5.0e-02 &   SM &   25.4 &  4.1 \\
  3539231 &   92.0 &  183.1 &        NaN &          planet &  1.7e-02 &  1.6e-03 &  5971 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    2.0 &  NaN \\
  3541946 &   17.8 &  146.9 &  K00624.01 &          planet &  2.7e-02 &  5.2e-04 &  5576 &     79 &   4.5 &  2.7e-02 &    0.9 &  4.1e-02 &   SM &    2.7 &  0.1 \\
  3547760 &    9.8 &  136.8 &        NaN &          Vshape &  1.2e-02 &  8.9e-04 &  5339 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.1 &  NaN \\
  3548044 &   68.0 &  163.6 &        NaN &          planet &  1.7e-02 &  1.2e-03 &  5725 &    130 &   4.3 &  3.1e-02 &    1.0 &  6.6e-02 &   SM &    2.0 &  0.2 \\
  3559935 &   29.9 &  134.9 &  K00492.01 &          planet &  2.7e-02 &  7.0e-04 &  5465 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    2.8 &  NaN \\
  3632089 &   31.8 &  136.8 &        NaN &          planet &  1.5e-02 &  8.1e-04 &  5683 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.6 &  NaN \\
  3642741 &    7.3 &  138.4 &  K00242.01 &          planet &  5.7e-02 &  1.1e-03 &  5546 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    5.3 &  NaN \\
  3655332 &   15.1 &  140.7 &  K01179.01 &        vardepth &  2.4e-01 &  1.2e-02 &  5818 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   25.3 &  NaN \\
  3657176 &   17.4 &  141.1 &  K02903.01 &  offset-no-star &  1.7e-02 &  9.7e-04 &  5887 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.8 &  NaN \\
  3728701 &   51.1 &  137.2 &  K02536.01 &          planet &  1.9e-02 &  1.9e-03 &  6054 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.3 &  NaN \\
  3732035 &  138.9 &  153.9 &        NaN &          planet &  2.3e-02 &  2.2e-03 &  6014 &    160 &   4.4 &  3.8e-02 &    1.1 &  3.5e-02 &   SM &    2.8 &  0.3 \\
  3745690 &   13.5 &  144.6 &  K00442.01 &          planet &  2.0e-02 &  1.3e-03 &  5768 &    150 &   4.4 &  1.1e-02 &    1.0 &  5.4e-02 &   SM &    2.2 &  0.2 \\
  3747817 &  184.8 &  217.4 &        NaN &          planet &  2.9e-02 &  2.7e-03 &  5275 &     74 &   4.6 &  1.5e-02 &    0.8 &  2.5e-02 &   SM &    2.5 &  0.2 \\
  3749134 &   11.3 &  134.9 &  K01212.01 &          planet &  1.6e-02 &  1.5e-03 &  5916 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.7 &  NaN \\
  3756264 &    7.4 &  136.9 &  K03108.01 &          planet &  2.0e-02 &  1.8e-03 &  5853 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.9 &  NaN \\
  3757588 &   24.1 &  154.3 &        NaN &         eclipse &  1.3e-01 &  4.9e-03 &  5386 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &   12.8 &  NaN \\
  3761319 &   16.2 &  143.9 &        NaN &          planet &  1.8e-02 &  1.1e-03 &  5758 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.9 &  NaN \\
  3833007 &   16.2 &  147.6 &  K00443.01 &          planet &  2.6e-02 &  9.8e-04 &  5891 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.5 &  NaN \\
  3835670 &   14.6 &  145.1 &  K00149.01 &          planet &  2.9e-02 &  8.1e-04 &  5724 &    151 &   4.1 &  2.6e-01 &    1.6 &  6.3e-01 &   SM &    5.0 &  2.0 \\
  3847138 &   11.7 &  142.2 &  K00444.01 &          planet &  2.0e-02 &  6.7e-04 &  5551 &     43 &   4.4 &  3.9e-02 &    0.9 &  3.5e-02 &   SM &    2.1 &  0.1 \\
  3848966 &   29.8 &  155.6 &        NaN &          planet &  1.4e-02 &  1.1e-03 &  6025 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.4 &  NaN \\
  3852655 &   11.6 &  132.8 &  K03002.01 &          planet &  9.1e-03 &  6.1e-04 &  5716 &    133 &   4.3 &  1.9e-01 &    1.2 &  3.1e-01 &   SM &    1.1 &  0.3 \\
  3858917 &   51.9 &  180.9 &        NaN &         eclipse &  9.8e-02 &  1.3e-03 &  5565 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    8.6 &  NaN \\
  3858949 &   26.0 &  154.9 &  K00995.01 &         eclipse &  2.8e-02 &  3.3e-04 &  5341 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.3 &  NaN \\
  3858988 &   26.0 &  154.8 &        NaN &         eclipse &  2.5e-02 &  3.5e-04 &  5738 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    2.9 &  NaN \\
  3859079 &   53.5 &  147.9 &  K01199.01 &          planet &  3.1e-02 &  2.3e-03 &  4385 &    128 &   4.7 &  4.3e-02 &    0.6 &  6.1e-02 &   SM &    2.0 &  0.3 \\
  3938073 &   31.0 &  158.9 &        NaN &         eclipse &  4.5e-01 &  4.1e-04 &  6007 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &   57.6 &  NaN \\
  3939150 &   17.3 &  142.1 &  K01215.01 &          planet &  1.4e-02 &  1.1e-03 &  6034 &    137 &   4.3 &  1.5e-01 &    1.3 &  2.4e-01 &   SM &    2.1 &  0.4 \\
  3942670 &   33.4 &  137.8 &  K00392.01 &          planet &  1.5e-02 &  3.3e-04 &  5989 &     79 &   4.3 &  1.5e-01 &    1.3 &  2.6e-01 &   SM &    2.1 &  0.4 \\
  3962872 &   26.0 &  148.8 &        NaN &          planet &  1.1e-02 &  4.4e-04 &  6055 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    1.3 &  NaN \\
  3966801 &   25.7 &  137.4 &  K00494.01 &          planet &  3.4e-02 &  2.2e-03 &  5055 &    -99 &   4.7 &      NaN &    0.7 &      NaN &    P &    2.6 &  NaN \\
  3969687 &   16.4 &  141.3 &  K02904.01 &          planet &  1.0e-02 &  8.9e-04 &  6049 &     53 &   4.1 &  1.5e-01 &    1.6 &  3.1e-01 &   SM &    1.8 &  0.4 \\
  3970233 &    8.3 &  133.1 &  K00604.01 &         eclipse &  1.2e-01 &  3.7e-05 &  5354 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   11.4 &  NaN \\
  4035640 &   28.3 &  140.9 &  K01881.01 &          planet &  3.1e-02 &  7.2e-04 &  5257 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.8 &  NaN \\
  4043190 &    6.4 &  136.9 &  K01220.01 &          planet &  1.1e-02 &  5.7e-04 &  5296 &    166 &   3.8 &  3.1e-01 &    2.5 &  9.9e-01 &   SM &    3.0 &  1.2 \\
  4043443 &  119.8 &  161.9 &  K00231.01 &          planet &  1.0e-01 &  1.4e-02 &  4604 &     32 &   4.7 &  4.5e-03 &    0.6 &  6.0e-03 &   SM &    7.4 &  1.0 \\
  4049901 &   16.3 &  132.1 &  K02295.01 &          planet &  6.4e-03 &  4.5e-04 &  5430 &     80 &   4.5 &  9.4e-03 &    0.8 &  2.3e-02 &   SM &    0.6 &  0.0 \\
  4075064 &   61.4 &  161.2 &        NaN &         eclipse &  6.9e-01 &  3.9e-02 &  4945 &    -99 &   4.7 &      NaN &    0.7 &      NaN &    P &   50.1 &  NaN \\
  4076976 &    9.8 &  133.7 &        NaN &          planet &  1.0e-02 &  4.3e-04 &  4960 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    0.8 &  NaN \\
  4077526 &   10.2 &  136.9 &  K01336.01 &          planet &  2.1e-02 &  1.2e-03 &  6082 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.5 &  NaN \\
  4077901 &   12.1 &  140.7 &        NaN &     offset-star &  1.0e-02 &  7.0e-04 &  5516 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    0.9 &  NaN \\
  4138008 &  112.3 &  230.5 &        NaN &          planet &  2.2e-02 &  2.8e-03 &  4402 &     69 &   4.7 &  1.4e-02 &    0.6 &  2.0e-02 &   SM &    1.4 &  0.2 \\
  4165473 &   13.0 &  139.5 &  K00550.01 &          planet &  2.2e-02 &  8.7e-04 &  5627 &     62 &   4.5 &  4.9e-02 &    1.0 &  4.7e-02 &   SM &    2.4 &  0.1 \\
  4172013 &   16.3 &  145.1 &  K02386.01 &          planet &  2.0e-02 &  1.5e-03 &  5877 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.9 &  NaN \\
  4178389 &   23.2 &  134.4 &  K00185.01 &          planet &  1.8e-01 &  6.7e-03 &  5927 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   18.0 &  NaN \\
  4242147 &   28.8 &  132.3 &  K01934.01 &          planet &  2.7e-02 &  1.0e-03 &  4569 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.8 &  NaN \\
  4247092 &   21.1 &  150.1 &  K00403.01 &          planet &  2.8e-02 &  1.5e-03 &  6160 &     37 &   4.4 &  2.8e-02 &    1.1 &  4.5e-02 &   SM &    3.5 &  0.2 \\
  4249725 &    6.3 &  132.7 &  K00222.01 &          planet &  3.3e-02 &  7.0e-04 &  4533 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    2.1 &  NaN \\
  4252322 &   14.6 &  137.1 &  K00396.01 &          planet &  3.2e-02 &  8.7e-04 &  5922 &    -99 &   4.2 &      NaN &    1.3 &      NaN &    P &    4.6 &  NaN \\
  4254466 &   42.3 &  168.8 &  K02134.01 &          planet &  2.2e-02 &  8.0e-04 &  5718 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.3 &  NaN \\
  4262581 &   37.6 &  161.5 &  K02122.01 &          planet &  1.9e-02 &  1.4e-03 &  5778 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.8 &  NaN \\
  4263529 &   10.1 &  132.9 &        NaN &          planet &  3.0e-02 &  1.1e-03 &  5520 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.7 &  NaN \\
  4270253 &   11.6 &  132.3 &  K00551.01 &          planet &  2.2e-02 &  1.1e-03 &  5841 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.1 &  NaN \\
  4276716 &   20.7 &  132.0 &  K01619.01 &          planet &  1.0e-02 &  1.2e-03 &  4882 &     72 &   4.6 &  5.3e-03 &    0.7 &  1.2e-02 &   SM &    0.8 &  0.1 \\
  4281895 &    9.5 &  137.8 &        NaN &         eclipse &  2.7e-01 &  9.1e-04 &  5608 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   28.7 &  NaN \\
  4352168 &   10.6 &  134.9 &        NaN &         eclipse &  6.3e-01 &  1.8e-03 &  5374 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   55.8 &  NaN \\
  4376644 &   27.7 &  146.1 &  K00397.01 &          Vshape &  1.5e-01 &  1.4e-02 &  6059 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   15.8 &  NaN \\
  4454934 &   33.5 &  140.2 &  K02245.01 &          planet &  1.8e-02 &  1.1e-03 &  5900 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    2.2 &  NaN \\
  4474462 &   12.9 &  141.9 &        NaN &          planet &  1.0e-02 &  1.0e-03 &  6050 &    -99 &   4.2 &      NaN &    1.4 &      NaN &    P &    1.6 &  NaN \\
  4478142 &  219.9 &  329.4 &        NaN &          planet &  2.5e-02 &  3.4e-03 &  5699 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.5 &  NaN \\
  4544907 &   46.9 &  137.7 &  K02024.01 &          planet &  2.3e-02 &  7.7e-04 &  5839 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.6 &  NaN \\
  4551663 &   12.1 &  140.5 &  K02576.01 &  offset-no-star &  1.4e-02 &  1.8e-03 &  5376 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  4552729 &   97.4 &  204.8 &  K02691.01 &          planet &  6.2e-02 &  9.9e-03 &  4704 &    -99 &   4.6 &      NaN &    0.6 &      NaN &    P &    4.4 &  NaN \\
  4563268 &    7.8 &  137.4 &  K00627.01 &          planet &  1.8e-02 &  5.8e-04 &  5999 &    110 &   4.2 &  1.3e-01 &    1.4 &  2.1e-01 &   SM &    2.9 &  0.4 \\
  4633570 &   16.7 &  141.3 &  K00446.01 &          planet &  2.6e-02 &  7.3e-04 &  4629 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.8 &  NaN \\
  4639868 &   53.1 &  136.0 &  K01326.01 &             ttv &  1.5e-01 &  1.7e-02 &  5467 &     88 &   4.4 &  4.8e-02 &    0.9 &  6.2e-02 &   SM &   15.0 &  2.1 \\
  4644604 &   14.5 &  131.6 &  K00628.01 &          planet &  2.0e-02 &  6.5e-04 &  5783 &    162 &   4.3 &  2.9e-02 &    1.1 &  6.3e-02 &   SM &    2.3 &  0.2 \\
  4644952 &    6.9 &  137.6 &  K01805.01 &          planet &  2.7e-02 &  1.3e-03 &  5529 &     74 &   4.5 &  3.0e-02 &    0.9 &  3.8e-02 &   SM &    2.6 &  0.2 \\
  4676964 &   43.1 &  140.1 &  K03069.01 &          planet &  1.7e-02 &  1.7e-03 &  5637 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.9 &  NaN \\
  4679314 &    7.7 &  133.3 &        NaN &        vardepth &  7.9e-03 &  3.1e-04 &  5747 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &    0.7 &  NaN \\
  4753988 &    7.3 &  135.0 &        NaN &         eclipse &  5.3e-01 &  1.9e-02 &  6039 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   54.4 &  NaN \\
  4773155 &   25.7 &  156.6 &        NaN &         eclipse &  6.5e-01 &  1.3e-03 &  5606 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   63.3 &  NaN \\
  4813563 &   36.5 &  151.3 &  K01959.01 &          planet &  2.7e-02 &  1.0e-03 &  4869 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.0 &  NaN \\
  4815520 &   31.6 &  145.7 &  K00367.01 &          planet &  4.2e-02 &  8.5e-04 &  5684 &     75 &   4.4 &  5.9e-02 &    1.1 &  7.8e-02 &   SM &    5.0 &  0.4 \\
  4820550 &  202.1 &  292.0 &        NaN &          planet &  5.7e-02 &  6.5e-03 &  5796 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    5.4 &  NaN \\
  4827723 &    7.2 &  135.0 &  K00632.01 &          planet &  1.5e-02 &  2.3e-04 &  5398 &     46 &   4.5 &  4.2e-02 &    0.9 &  4.1e-02 &   SM &    1.4 &  0.1 \\
  4833421 &   12.5 &  134.0 &  K00232.01 &          planet &  4.6e-02 &  1.2e-03 &  6063 &    139 &   4.4 &  3.8e-02 &    1.1 &  4.2e-02 &   SM &    5.6 &  0.3 \\
  4841374 &  161.5 &  170.6 &  K00633.01 &          planet &  2.7e-02 &  1.8e-03 &  5758 &    143 &   4.4 &  5.2e-02 &    1.0 &  6.7e-02 &   SM &    3.0 &  0.3 \\
  4847534 &    9.7 &  135.9 &  K00499.01 &          planet &  1.9e-02 &  7.3e-04 &  5214 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.7 &  NaN \\
  4847832 &   31.0 &  139.4 &        NaN &          Vshape &  6.0e-01 &  1.2e-03 &  5186 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   52.3 &  NaN \\
  4857058 &    7.3 &  132.1 &  K03061.01 &          planet &  1.3e-02 &  1.1e-03 &  5062 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.0 &  NaN \\
  4860678 &   10.0 &  137.3 &  K01602.01 &          planet &  1.5e-02 &  1.3e-03 &  5813 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.4 &  NaN \\
  4860932 &   12.4 &  137.9 &  K01600.01 &        vardepth &  1.8e-02 &  7.9e-04 &  6059 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.8 &  NaN \\
  4912650 &  100.3 &  152.8 &        NaN &          planet &  1.7e-02 &  1.9e-03 &  5180 &     36 &   4.5 &  3.2e-02 &    0.8 &  3.5e-02 &   SM &    1.5 &  0.2 \\
  4932442 &    6.9 &  137.1 &  K01665.01 &          planet &  1.0e-02 &  7.1e-04 &  5869 &     96 &   4.2 &  1.4e-01 &    1.4 &  2.5e-01 &   SM &    1.6 &  0.3 \\
  4948730 &   23.0 &  139.9 &        NaN &         eclipse &  2.2e-02 &  1.8e-03 &  5876 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.4 &  NaN \\
  4949751 &   31.8 &  154.6 &  K00404.01 &          Vshape &  9.9e-02 &  4.5e-03 &  5956 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    9.9 &  NaN \\
  4951877 &   24.8 &  145.5 &  K00501.01 &          planet &  2.2e-02 &  7.5e-04 &  5750 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.1 &  NaN \\
  4989057 &    7.2 &  137.7 &  K01923.01 &          planet &  2.0e-02 &  1.3e-03 &  5416 &     33 &   4.5 &  1.3e-02 &    0.9 &  1.2e-02 &   SM &    1.9 &  0.1 \\
  5003117 &   37.6 &  153.1 &  K00405.01 &         eclipse &  1.5e-01 &  4.0e-04 &  5576 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   14.2 &  NaN \\
  5025294 &    5.5 &  134.3 &        NaN &         eclipse &  7.3e-02 &  2.5e-02 &  5978 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    7.5 &  NaN \\
  5035972 &   49.3 &  141.9 &  K00406.01 &         eclipse &  1.5e-01 &  3.4e-03 &  5848 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   16.7 &  NaN \\
  5042210 &   12.1 &  131.6 &  K02462.01 &          planet &  7.6e-03 &  2.3e-04 &  5995 &    111 &   4.3 &  1.5e-01 &    1.3 &  2.5e-01 &   SM &    1.1 &  0.2 \\
  5088591 &   14.5 &  140.7 &  K01801.01 &          planet &  3.5e-02 &  1.1e-03 &  5331 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.2 &  NaN \\
  5091614 &   21.1 &  138.4 &        NaN &         eclipse &  4.0e-01 &  1.4e-03 &  6077 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   42.5 &  NaN \\
  5095082 &   20.7 &  145.6 &        NaN &          planet &  8.8e-03 &  6.6e-04 &  5520 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    0.9 &  NaN \\
  5096590 &   29.6 &  137.3 &  K03093.01 &          planet &  1.0e-02 &  7.4e-04 &  5818 &     98 &   4.3 &  1.7e-01 &    1.2 &  2.6e-01 &   SM &    1.3 &  0.3 \\
  5098444 &   26.9 &  151.0 &  K00637.01 &         eclipse &  1.4e-01 &  8.9e-04 &  4918 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   10.6 &  NaN \\
  5103942 &   10.1 &  131.8 &        NaN &          planet &  2.2e-02 &  1.6e-03 &  6090 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.3 &  NaN \\
  5113822 &   23.6 &  149.0 &  K00638.01 &          planet &  3.1e-02 &  3.5e-03 &  5685 &    118 &   4.4 &  5.3e-02 &    1.0 &  7.8e-02 &   SM &    3.2 &  0.5 \\
  5121511 &   31.0 &  160.8 &  K00640.01 &          planet &  2.4e-02 &  5.7e-04 &  5216 &     69 &   4.5 &  2.1e-02 &    0.8 &  1.3e-02 &   SM &    2.2 &  0.1 \\
  5128673 &   88.0 &  168.3 &  K02698.01 &          planet &  3.0e-02 &  2.0e-03 &  5845 &     55 &   4.3 &  1.1e-01 &    1.2 &  1.7e-01 &   SM &    3.9 &  0.6 \\
  5131180 &   14.9 &  133.4 &  K00641.01 &  offset-no-star &  3.0e-02 &  1.5e-03 &  4240 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.8 &  NaN \\
  5193077 &   22.3 &  146.4 &        NaN &     offset-star &  9.0e-03 &  5.0e-04 &  5785 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    0.9 &  NaN \\
  5199426 &   78.6 &  144.0 &        NaN &          Vshape &  3.6e-01 &  3.9e-02 &  5946 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   38.9 &  NaN \\
  5213404 &   20.7 &  140.0 &        NaN &          planet &  1.2e-02 &  1.2e-03 &  5793 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.3 &  NaN \\
  5217586 &   26.1 &  143.1 &  K01592.01 &          planet &  2.5e-02 &  2.8e-04 &  5614 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.8 &  NaN \\
  5254230 &    7.0 &  137.9 &        NaN &         eclipse &  4.2e-02 &  1.4e-02 &  5369 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    4.0 &  NaN \\
  5266937 &    5.9 &  132.9 &        NaN &         eclipse &  6.2e-01 &  3.9e-04 &  5655 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   67.7 &  NaN \\
  5272233 &    9.0 &  133.6 &  K02711.01 &          planet &  1.4e-02 &  7.5e-04 &  5823 &     91 &   4.3 &  1.6e-01 &    1.2 &  2.4e-01 &   SM &    1.7 &  0.4 \\
  5282051 &    5.9 &  135.7 &  K00502.01 &     offset-star &  1.4e-02 &  4.9e-04 &  5546 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.5 &  NaN \\
  5299459 &   10.4 &  132.6 &  K01576.01 &          planet &  2.6e-02 &  3.8e-04 &  5489 &     70 &   4.4 &  6.6e-02 &    1.0 &  7.4e-02 &   SM &    2.8 &  0.2 \\
  5301750 &    8.7 &  138.8 &  K01589.01 &          planet &  2.0e-02 &  7.5e-04 &  6094 &    104 &   4.4 &  2.9e-02 &    1.1 &  3.8e-02 &   SM &    2.4 &  0.1 \\
  5303346 &   37.3 &  143.0 &        NaN &         eclipse &  1.2e-01 &  2.1e-03 &  5297 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    9.9 &  NaN \\
  5308537 &   14.3 &  143.2 &        NaN &          planet &  7.8e-03 &  7.0e-04 &  5896 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    0.8 &  NaN \\
  5340644 &    8.2 &  131.8 &  K00503.01 &          planet &  3.5e-02 &  1.6e-03 &  4272 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    2.1 &  NaN \\
  5351250 &    7.4 &  136.2 &  K00408.01 &          planet &  3.5e-02 &  1.1e-03 &  5554 &     94 &   4.5 &  2.8e-02 &    0.9 &  3.9e-02 &   SM &    3.4 &  0.2 \\
  5360082 &   11.4 &  133.3 &        NaN &         eclipse &  1.3e-01 &  7.4e-04 &  4723 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    9.0 &  NaN \\
  5374403 &   40.8 &  152.8 &  K02556.01 &          planet &  1.4e-02 &  7.8e-04 &  5523 &     21 &   4.5 &  5.6e-02 &    0.9 &  5.1e-02 &   SM &    1.4 &  0.1 \\
  5375194 &   13.5 &  142.2 &  K01825.01 &          planet &  2.3e-02 &  6.2e-04 &  5337 &     48 &   4.6 &  7.4e-03 &    0.8 &  1.8e-02 &   SM &    2.1 &  0.1 \\
  5393558 &   10.2 &  137.3 &        NaN &         eclipse &  6.3e-01 &  6.1e-03 &  5888 &    -99 &   4.2 &      NaN &    1.3 &      NaN &    P &   89.0 &  NaN \\
  5431027 &    8.8 &  136.9 &        NaN &          planet &  1.1e-02 &  1.1e-03 &  5596 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    1.3 &  NaN \\
  5438757 &   10.4 &  133.7 &  K01601.01 &          planet &  1.5e-02 &  3.6e-04 &  5727 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &    1.4 &  NaN \\
  5443604 &   21.4 &  141.3 &  K02713.01 &        vardepth &  2.2e-02 &  3.3e-03 &  4896 &    -99 &   4.7 &      NaN &    0.7 &      NaN &    P &    1.6 &  NaN \\
  5444548 &   13.2 &  139.8 &  K00409.01 &          planet &  2.4e-02 &  1.2e-03 &  5796 &     67 &   4.4 &  6.4e-02 &    1.1 &  8.6e-02 &   SM &    3.0 &  0.3 \\
  5446285 &   10.9 &  134.8 &  K00142.01 &             ttv &  5.1e-04 &  3.6e-03 &  5423 &     36 &   4.5 &  1.2e-02 &    0.9 &  2.2e-02 &   SM &    0.0 &  0.4 \\
  5461440 &   40.6 &  158.7 &  K00504.01 &          planet &  2.4e-02 &  1.9e-03 &  5579 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
  5474613 &   20.4 &  140.1 &  K01599.01 &          planet &  1.6e-02 &  7.9e-04 &  5762 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.6 &  NaN \\
  5478055 &   15.9 &  142.5 &  K00411.01 &        vardepth &  2.2e-02 &  7.3e-04 &  5982 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &    2.8 &  NaN \\
  5480640 &   58.0 &  138.8 &  K02707.01 &          planet &  2.7e-02 &  1.5e-03 &  5610 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.4 &  NaN \\
  5481148 &   22.0 &  135.2 &  K02701.01 &     offset-star &  3.8e-02 &  1.3e-03 &  5836 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.7 &  NaN \\
  5520547 &   11.2 &  137.5 &  K02990.01 &          planet &  1.4e-02 &  8.0e-04 &  6055 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.5 &  NaN \\
  5526527 &   16.7 &  143.1 &  K01838.01 &          planet &  3.1e-02 &  9.4e-04 &  4565 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    2.1 &  NaN \\
  5526717 &   52.1 &  178.2 &  K01677.01 &          planet &  2.2e-02 &  1.6e-03 &  5717 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
  5530882 &    5.1 &  132.9 &  K01680.01 &     offset-star &  8.8e-03 &  6.1e-04 &  5709 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    0.8 &  NaN \\
  5535280 &   75.0 &  146.1 &        NaN &         eclipse &  4.1e-01 &  4.2e-02 &  5950 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   41.0 &  NaN \\
  5546277 &    7.5 &  137.4 &        NaN &         eclipse &  2.4e-02 &  4.6e-04 &  5809 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.3 &  NaN \\
  5546761 &   17.7 &  131.6 &  K02160.01 &          planet &  1.6e-02 &  9.0e-04 &  5807 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.5 &  NaN \\
  5553624 &   25.8 &  150.6 &        NaN &          Vshape &  5.3e-01 &  9.4e-03 &  5545 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   48.1 &  NaN \\
  5562784 &   25.3 &  142.2 &  K00608.01 &        vardepth &  5.1e-02 &  5.0e-04 &  4502 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    3.3 &  NaN \\
  5563300 &   71.1 &  134.8 &        NaN &          Vshape &  7.3e-02 &  9.8e-03 &  5272 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    6.7 &  NaN \\
  5640085 &   10.1 &  137.9 &  K00448.01 &          planet &  3.3e-02 &  1.9e-03 &  4616 &     28 &   4.6 &  1.3e-02 &    0.7 &  1.4e-02 &   SM &    2.4 &  0.1 \\
  5652010 &   14.6 &  140.3 &        NaN &          planet &  9.9e-03 &  9.9e-04 &  5399 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.0 &  NaN \\
  5686174 &   14.3 &  138.0 &  K00610.01 &          planet &  3.2e-02 &  2.7e-03 &  4207 &    -99 &   4.7 &      NaN &    0.5 &      NaN &    P &    1.9 &  NaN \\
  5700330 &   53.2 &  181.7 &        NaN &          planet &  7.4e-02 &  4.2e-04 &  5883 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &    9.8 &  NaN \\
  5702939 &   18.4 &  144.9 &  K03000.01 &  offset-no-star &  1.1e-02 &  4.1e-04 &  5606 &    170 &   4.4 &  4.8e-02 &    1.0 &  6.6e-02 &   SM &    1.2 &  0.1 \\
  5706966 &   12.6 &  137.3 &  K01908.01 &          planet &  2.1e-02 &  1.2e-03 &  4350 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.3 &  NaN \\
  5709725 &   86.5 &  181.9 &  K00555.02 &          planet &  2.9e-02 &  2.1e-03 &  5246 &     77 &   4.5 &  1.9e-02 &    0.8 &  1.8e-02 &   SM &    2.6 &  0.2 \\
  5728139 &    5.3 &  132.0 &  K00206.01 &          planet &  6.3e-02 &  4.6e-04 &  6043 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    7.8 &  NaN \\
  5731312 &    7.9 &  135.1 &        NaN &          Vshape &  4.8e-01 &  8.2e-03 &  4938 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   37.1 &  NaN \\
  5735762 &    9.7 &  135.0 &  K00148.02 &          planet &  2.8e-02 &  3.3e-04 &  5203 &     61 &   4.5 &  2.7e-02 &    0.8 &  3.3e-02 &   SM &    2.5 &  0.1 \\
  5738496 &    9.5 &  137.7 &  K00556.01 &         eclipse &  1.9e-02 &  8.7e-04 &  5921 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.9 &  NaN \\
  5768816 &   48.0 &  160.7 &        NaN &          planet &  2.4e-02 &  6.0e-04 &  5613 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.5 &  NaN \\
  5770074 &   63.0 &  169.1 &  K01928.01 &          planet &  2.4e-02 &  1.3e-03 &  5804 &    105 &   4.4 &  4.7e-02 &    1.1 &  6.4e-02 &   SM &    2.7 &  0.2 \\
  5771719 &   12.3 &  139.3 &  K00190.01 &          planet &  1.1e-01 &  4.6e-04 &  5538 &    -99 &   4.1 &      NaN &    1.4 &      NaN &    P &   16.9 &  NaN \\
  5774349 &   15.7 &  139.5 &  K00557.01 &          planet &  3.5e-02 &  1.1e-03 &  5147 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.9 &  NaN \\
  5780930 &   16.8 &  131.6 &        NaN &          planet &  1.7e-02 &  6.7e-04 &  4683 &    -99 &   4.6 &      NaN &    0.6 &      NaN &    P &    1.2 &  NaN \\
  5781192 &    9.5 &  138.3 &        NaN &         eclipse &  6.9e-01 &  8.1e-03 &  5539 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   60.6 &  NaN \\
  5786676 &   12.0 &  142.9 &  K00650.01 &          planet &  2.6e-02 &  9.8e-04 &  5064 &     56 &   4.6 &  1.7e-02 &    0.8 &  2.4e-02 &   SM &    2.2 &  0.1 \\
  5791986 &   15.2 &  146.1 &  K00413.01 &          planet &  3.1e-02 &  9.3e-04 &  5439 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.7 &  NaN \\
  5794570 &    5.4 &  132.5 &  K02675.01 &          planet &  2.3e-02 &  1.6e-03 &  5693 &     99 &   4.5 &  3.7e-02 &    1.0 &  5.5e-02 &   SM &    2.4 &  0.2 \\
  5796675 &   16.1 &  134.5 &  K00652.01 &          planet &  5.4e-02 &  1.0e-03 &  5305 &     87 &   4.5 &  1.8e-02 &    0.8 &  2.4e-02 &   SM &    4.9 &  0.2 \\
  5807769 &    8.0 &  132.3 &        NaN &          planet &  1.3e-02 &  8.6e-04 &  5948 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  5812960 &   18.5 &  136.5 &  K00507.01 &          planet &  3.7e-02 &  1.0e-03 &  5290 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    3.4 &  NaN \\
  5819801 &   11.8 &  138.3 &        NaN &          planet &  5.7e-03 &  3.7e-04 &  5522 &    -99 &   4.1 &      NaN &    1.4 &      NaN &    P &    0.9 &  NaN \\
  5866099 &   37.0 &  133.6 &  K01055.01 &         eclipse &  6.3e-02 &  3.7e-03 &  5571 &    -99 &   4.1 &      NaN &    1.4 &      NaN &    P &    9.6 &  NaN \\
  5872150 &   20.4 &  134.6 &  K00414.01 &         eclipse &  1.4e-01 &  1.7e-04 &  6041 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   16.3 &  NaN \\
  5903749 &   19.0 &  134.8 &  K03029.01 &          planet &  1.8e-02 &  1.2e-03 &  5421 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.8 &  NaN \\
  5906426 &   13.9 &  143.5 &  K02377.01 &          planet &  1.8e-02 &  1.8e-03 &  5229 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.6 &  NaN \\
  5940165 &    9.3 &  140.4 &  K02031.01 &          planet &  3.8e-02 &  5.4e-03 &  4452 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    2.4 &  NaN \\
  5941160 &    8.6 &  137.3 &  K00654.01 &          planet &  1.7e-02 &  7.6e-04 &  5662 &     96 &   4.5 &  3.9e-02 &    0.9 &  4.1e-02 &   SM &    1.7 &  0.1 \\
  5953297 &    5.6 &  132.9 &  K02733.01 &          planet &  1.3e-02 &  3.7e-04 &  4809 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    0.9 &  NaN \\
  5959719 &    6.7 &  133.3 &  K02498.01 &          planet &  9.2e-03 &  1.1e-03 &  5153 &     49 &   4.6 &  3.0e-02 &    0.8 &  2.7e-02 &   SM &    0.8 &  0.1 \\
  5959753 &    8.3 &  138.1 &  K00226.01 &          planet &  2.6e-02 &  7.2e-04 &  5241 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.1 &  NaN \\
  5966322 &   60.9 &  173.4 &  K00303.01 &          planet &  2.5e-02 &  6.0e-04 &  5560 &     46 &   4.4 &  2.8e-02 &    0.9 &  3.1e-02 &   SM &    2.5 &  0.1 \\
  5972334 &   15.4 &  132.4 &  K00191.01 &          planet &  1.1e-01 &  6.5e-04 &  5417 &     76 &   4.5 &  2.6e-02 &    0.9 &  1.5e-02 &   SM &   10.7 &  0.2 \\
  5978361 &    9.2 &  136.4 &  K00558.01 &          planet &  2.6e-02 &  1.3e-03 &  5505 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.2 &  NaN \\
  5992270 &   58.4 &  168.3 &        NaN &  offset-no-star &  5.7e-02 &  1.6e-02 &  4386 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    3.6 &  NaN \\
  6029130 &   12.6 &  134.7 &        NaN &         eclipse &  7.5e-01 &  1.1e-01 &  5289 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   60.4 &  NaN \\
  6034945 &    9.1 &  134.0 &  K01683.01 &          planet &  1.7e-02 &  9.6e-04 &  5919 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.9 &  NaN \\
  6037187 &   41.8 &  142.8 &  K01061.01 &          planet &  2.1e-02 &  1.3e-03 &  5899 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.2 &  NaN \\
  6037581 &    9.6 &  136.6 &  K01916.02 &          planet &  1.6e-02 &  7.7e-04 &  5865 &     70 &   4.4 &  5.9e-02 &    1.1 &  7.4e-02 &   SM &    1.9 &  0.2 \\
  6046540 &    7.3 &  134.4 &  K00200.01 &          planet &  8.2e-02 &  5.4e-04 &  5940 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    8.2 &  NaN \\
  6058816 &   73.7 &  188.5 &        NaN &          planet &  1.4e-02 &  9.2e-04 &  6093 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.5 &  NaN \\
  6072593 &    5.1 &  133.9 &  K03070.01 &     offset-star &  1.0e-02 &  9.6e-04 &  5914 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    1.2 &  NaN \\
  6119141 &   29.1 &  137.0 &  K02343.01 &          planet &  1.9e-02 &  1.0e-03 &  5781 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.2 &  NaN \\
  6124512 &    8.4 &  134.4 &  K02627.01 &          planet &  9.5e-03 &  6.0e-04 &  5469 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.0 &  NaN \\
  6131659 &   17.5 &  144.6 &        NaN &         eclipse &  5.7e-01 &  9.7e-04 &  5088 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   46.9 &  NaN \\
  6137704 &  178.3 &  255.3 &        NaN &          Vshape &  2.8e-01 &  2.8e-02 &  5195 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   24.8 &  NaN \\
  6142862 &    5.3 &  133.4 &  K02336.01 &     offset-star &  1.4e-02 &  1.1e-03 &  4423 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    0.9 &  NaN \\
  6146418 &   22.4 &  149.1 &        NaN &         eclipse &  7.5e-02 &  9.0e-04 &  6077 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &    9.8 &  NaN \\
  6146838 &   27.5 &  143.7 &        NaN &          radius &  2.4e-01 &  3.9e-04 &  5600 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &   24.2 &  NaN \\
  6147573 &   25.8 &  137.4 &        NaN &         eclipse &  4.0e-01 &  7.3e-03 &  5695 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   40.3 &  NaN \\
  6152974 &   20.2 &  141.2 &  K00216.01 &          planet &  7.1e-02 &  3.5e-03 &  5187 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    6.1 &  NaN \\
  6184894 &    7.2 &  135.2 &        NaN &          planet &  3.8e-02 &  9.9e-04 &  5485 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    3.5 &  NaN \\
  6185476 &   17.7 &  136.0 &  K00227.01 &             ttv &  9.3e-03 &  1.5e-03 &  4264 &     84 &   4.7 &  1.2e-02 &    0.5 &  6.2e-02 &   SM &    0.5 &  0.1 \\
  6185711 &   11.7 &  139.4 &  K00169.01 &        vardepth &  2.0e-02 &  5.3e-04 &  5814 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.9 &  NaN \\
  6209677 &    7.8 &  138.1 &  K01750.01 &          planet &  1.3e-02 &  6.2e-04 &  5799 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.4 &  NaN \\
  6225454 &   89.3 &  218.5 &        NaN &          planet &  2.4e-02 &  5.8e-03 &  4549 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.6 &  NaN \\
  6266741 &    7.9 &  137.8 &  K00508.01 &          planet &  2.6e-02 &  8.6e-04 &  5614 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    3.3 &  NaN \\
  6267535 &    6.1 &  134.1 &  K00660.01 &          planet &  1.6e-02 &  9.0e-04 &  5317 &    183 &   3.9 &  4.2e-01 &    2.1 &  1.0e+00 &   SM &    3.7 &  1.9 \\
  6289650 &  166.8 &  245.1 &  K00415.01 &          planet &  6.4e-02 &  3.3e-03 &  5663 &    149 &   4.4 &  3.1e-02 &    1.0 &  7.2e-02 &   SM &    7.0 &  0.6 \\
  6305192 &    8.0 &  132.5 &  K00219.01 &          planet &  5.3e-02 &  7.9e-04 &  6006 &    111 &   4.2 &  1.3e-01 &    1.5 &  2.1e-01 &   SM &    8.4 &  1.2 \\
  6307062 &   75.4 &  167.1 &        NaN &         eclipse &  8.8e-01 &  6.0e-02 &  5416 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   74.7 &  NaN \\
  6307063 &  376.9 &  317.9 &        NaN &         eclipse &  3.3e-02 &  1.3e-02 &  5872 &     94 &   4.4 &  6.2e-02 &    1.1 &  8.2e-02 &   SM &    4.0 &  1.6 \\
  6307083 &   75.4 &  167.1 &        NaN &         eclipse &  1.7e-02 &  9.3e-04 &  5047 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.4 &  NaN \\
  6342333 &   80.2 &  162.4 &        NaN &          planet &  3.1e-02 &  4.0e-03 &  5655 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.0 &  NaN \\
  6346809 &   17.6 &  137.7 &  K02775.01 &          planet &  2.1e-02 &  1.4e-03 &  5681 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    2.2 &  NaN \\
  6347299 &   14.4 &  131.8 &  K00661.01 &          planet &  1.8e-02 &  5.4e-04 &  5789 &     27 &   4.4 &  1.3e-01 &    1.1 &  2.0e-01 &   SM &    2.2 &  0.4 \\
  6351097 &   12.5 &  136.3 &  K02618.01 &  offset-no-star &  1.3e-02 &  1.1e-03 &  5771 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  6356692 &   11.4 &  141.6 &  K02948.01 &          planet &  6.5e-03 &  4.2e-04 &  5561 &     46 &   4.2 &  1.2e-01 &    1.4 &  1.9e-01 &   SM &    1.0 &  0.2 \\
  6359798 &   14.2 &  140.7 &  K01121.01 &         eclipse &  3.6e-01 &  3.7e-03 &  5855 &     86 &   4.4 &  6.4e-02 &    1.1 &  8.7e-02 &   SM &   42.4 &  3.5 \\
  6364582 &   30.9 &  200.0 &        NaN &          planet &  1.2e-02 &  1.8e-04 &  6012 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    1.4 &  NaN \\
  6383821 &   27.1 &  139.1 &  K01238.01 &          planet &  2.2e-02 &  9.9e-04 &  5611 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.0 &  NaN \\
  6421188 &   16.4 &  136.3 &        NaN &         eclipse &  2.0e-01 &  4.5e-04 &  5948 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &   24.8 &  NaN \\
  6428794 &  169.1 &  201.8 &        NaN &          planet &  2.5e-02 &  2.8e-03 &  5172 &     23 &   4.5 &  3.2e-02 &    0.8 &  3.4e-02 &   SM &    2.2 &  0.3 \\
  6432345 &  234.6 &  172.6 &  K02757.01 &          planet &  2.8e-02 &  2.7e-03 &  5421 &     71 &   4.5 &  2.7e-02 &    0.9 &  1.5e-02 &   SM &    2.7 &  0.3 \\
  6442340 &   13.1 &  144.0 &  K00664.01 &          planet &  1.5e-02 &  8.2e-04 &  5717 &     93 &   4.4 &  4.9e-02 &    1.1 &  6.1e-02 &   SM &    1.7 &  0.1 \\
  6449552 &   20.1 &  135.8 &        NaN &         eclipse &  7.0e-01 &  5.5e-04 &  5524 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &   69.9 &  NaN \\
  6468138 &  134.3 &  182.7 &  K01826.01 &          planet &  2.7e-02 &  1.7e-03 &  5807 &     48 &   4.4 &  6.3e-02 &    1.0 &  6.9e-02 &   SM &    3.0 &  0.3 \\
  6468938 &    7.2 &  135.5 &        NaN &         eclipse &  4.0e-01 &  1.2e-02 &  6068 &    -99 &   4.2 &      NaN &    1.3 &      NaN &    P &   57.0 &  NaN \\
  6471021 &  125.6 &  253.3 &  K00372.01 &          planet &  7.9e-02 &  1.1e-03 &  5623 &     77 &   4.4 &  3.6e-02 &    0.9 &  4.8e-02 &   SM &    8.0 &  0.4 \\
  6500206 &   13.4 &  142.4 &  K02451.01 &          planet &  2.2e-02 &  1.9e-03 &  5315 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.0 &  NaN \\
  6501635 &   23.7 &  131.9 &  K00560.01 &          planet &  2.8e-02 &  1.0e-03 &  5277 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.3 &  NaN \\
  6504534 &   28.2 &  143.7 &        NaN &          planet &  2.0e-01 &  2.3e-03 &  4909 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   14.9 &  NaN \\
  6508221 &   18.2 &  149.4 &  K00416.01 &          planet &  3.6e-02 &  2.2e-04 &  5085 &     78 &   4.6 &  3.2e-02 &    0.7 &  3.8e-02 &   SM &    2.9 &  0.2 \\
  6521045 &   12.8 &  135.8 &  K00041.01 &          planet &  1.3e-02 &  1.8e-04 &  5846 &    129 &   4.3 &  1.3e-01 &    1.3 &  2.0e-01 &   SM &    1.9 &  0.3 \\
  6522750 &   17.4 &  135.7 &        NaN &         eclipse &  7.8e-01 &  1.1e-02 &  5802 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   80.1 &  NaN \\
  6523351 &    6.1 &  136.1 &  K03117.01 &          planet &  7.8e-03 &  8.8e-04 &  5544 &     97 &   4.5 &  2.9e-02 &    0.9 &  4.3e-02 &   SM &    0.8 &  0.1 \\
  6525209 &   75.1 &  200.8 &        NaN &          planet &  1.9e-01 &  8.6e-04 &  5421 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   16.1 &  NaN \\
  6541920 &   32.0 &  154.2 &  K00157.03 &          planet &  3.4e-02 &  8.0e-04 &  5796 &     43 &   4.4 &  3.7e-02 &    1.0 &  3.5e-02 &   SM &    3.8 &  0.2 \\
  6584273 &   51.1 &  143.8 &        NaN &          planet &  2.0e-02 &  2.0e-03 &  5979 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.0 &  NaN \\
  6587002 &   47.4 &  169.1 &  K00612.02 &          planet &  2.7e-02 &  1.2e-03 &  5124 &     23 &   4.5 &  2.8e-02 &    0.8 &  3.4e-02 &   SM &    2.4 &  0.1 \\
  6594972 &   10.8 &  133.0 &        NaN &         eclipse &  8.2e-01 &  1.4e-02 &  5957 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   89.9 &  NaN \\
  6607357 &    7.7 &  134.4 &  K02838.01 &          planet &  8.5e-03 &  9.7e-04 &  5731 &     35 &   4.3 &  2.2e-02 &    1.2 &  2.6e-02 &   SM &    1.1 &  0.1 \\
  6613006 &    7.4 &  133.9 &  K01223.01 &         eclipse &  1.2e-01 &  1.5e-04 &  5858 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   11.4 &  NaN \\
  6634112 &    9.9 &  133.9 &        NaN &          Vshape &  1.9e-01 &  3.4e-03 &  5253 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   16.9 &  NaN \\
  6634133 &    9.9 &  133.9 &        NaN &        vardepth &  1.7e-02 &  9.2e-04 &  5123 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.4 &  NaN \\
  6665223 &  119.4 &  232.6 &  K01232.01 &          planet &  1.7e-01 &  2.1e-02 &  5317 &      8 &   4.5 &  3.5e-02 &    0.9 &  4.3e-02 &   SM &   16.2 &  2.1 \\
  6665512 &    6.9 &  135.6 &  K02005.01 &          planet &  2.2e-02 &  1.2e-03 &  4559 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.4 &  NaN \\
  6665695 &    5.4 &  132.0 &  K00561.01 &          planet &  2.0e-02 &  9.9e-04 &  5072 &     66 &   4.6 &  3.8e-02 &    0.8 &  4.7e-02 &   SM &    1.7 &  0.1 \\
  6685609 &    5.9 &  135.1 &  K00665.01 &          planet &  2.0e-02 &  8.6e-04 &  5923 &    121 &   4.2 &  1.6e-01 &    1.5 &  2.9e-01 &   SM &    3.2 &  0.7 \\
  6692833 &   10.8 &  134.1 &  K01244.01 &  offset-no-star &  1.6e-02 &  1.6e-03 &  6075 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.7 &  NaN \\
  6694186 &    5.6 &  135.2 &        NaN &         eclipse &  3.4e-01 &  2.5e-04 &  5458 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &   35.1 &  NaN \\
  6705137 &    5.6 &  131.9 &  K02609.01 &     offset-star &  1.3e-02 &  1.2e-03 &  5799 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.2 &  NaN \\
  6707835 &   22.2 &  151.9 &  K00666.01 &          planet &  2.3e-02 &  7.9e-04 &  5615 &     79 &   4.4 &  5.6e-02 &    1.0 &  6.5e-02 &   SM &    2.5 &  0.2 \\
  6751874 &    6.9 &  132.5 &  K02282.01 &          planet &  1.5e-02 &  1.6e-03 &  6054 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.6 &  NaN \\
  6752002 &    6.1 &  136.9 &        NaN &          planet &  1.1e-02 &  1.5e-03 &  4936 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    0.9 &  NaN \\
  6761777 &   47.3 &  146.3 &        NaN &          planet &  1.7e-02 &  1.1e-03 &  6005 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.8 &  NaN \\
  6762829 &   18.8 &  138.7 &        NaN &         eclipse &  1.5e-01 &  2.7e-05 &  5898 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   15.8 &  NaN \\
  6786037 &   21.1 &  150.8 &  K00564.01 &          planet &  2.3e-02 &  1.0e-03 &  5951 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.3 &  NaN \\
  6803202 &   21.1 &  143.6 &  K00177.01 &          planet &  1.6e-02 &  6.8e-04 &  5711 &    110 &   4.4 &  4.0e-02 &    1.0 &  5.9e-02 &   SM &    1.8 &  0.1 \\
  6838050 &    6.5 &  133.9 &  K00512.01 &          planet &  2.3e-02 &  1.3e-03 &  5488 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.4 &  NaN \\
  6841577 &   15.5 &  140.3 &        NaN &         eclipse &  4.6e-01 &  4.9e-04 &  5741 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   45.7 &  NaN \\
  6842682 &    7.6 &  135.6 &  K02649.01 &          planet &  1.4e-02 &  1.0e-03 &  5820 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  6846911 &   14.0 &  135.2 &  K02477.01 &          planet &  2.0e-02 &  1.8e-03 &  5911 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.4 &  NaN \\
  6850504 &   10.9 &  138.6 &  K00070.01 &          planet &  3.5e-02 &  5.3e-04 &  5521 &    109 &   4.5 &  3.5e-02 &    0.9 &  4.1e-02 &   SM &    3.4 &  0.2 \\
  6851425 &   11.1 &  139.7 &  K00163.01 &          planet &  2.3e-02 &  4.4e-04 &  5079 &     92 &   4.6 &  2.6e-02 &    0.7 &  3.4e-02 &   SM &    1.8 &  0.1 \\
  6864893 &   40.9 &  163.4 &  K02375.01 &         eclipse &  1.8e-02 &  1.4e-03 &  5441 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.5 &  NaN \\
  6871071 &    5.0 &  134.1 &  K02220.02 &          planet &  1.3e-02 &  8.1e-04 &  6023 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.3 &  NaN \\
  6879865 &   19.2 &  138.6 &  K00417.01 &          planet &  1.0e-01 &  2.6e-02 &  5867 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    9.8 &  NaN \\
  6922203 &   13.3 &  133.8 &  K02578.01 &          planet &  2.3e-02 &  2.2e-03 &  5992 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.7 &  NaN \\
  6924203 &    6.9 &  135.3 &  K01370.01 &          planet &  2.0e-02 &  1.2e-03 &  5704 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.8 &  NaN \\
  6934986 &  131.5 &  177.5 &  K02294.01 &          planet &  2.7e-02 &  7.2e-03 &  5755 &     58 &   4.2 &  1.3e-01 &    1.4 &  2.2e-01 &   SM &    4.1 &  1.3 \\
  6936977 &   36.5 &  159.8 &        NaN &          radius &  4.1e-01 &  4.1e-03 &  5468 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   35.4 &  NaN \\
  6947164 &   70.6 &  190.5 &        NaN &          radius &  5.3e-01 &  2.4e-02 &  5976 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   53.8 &  NaN \\
  6960445 &    5.1 &  136.0 &  K00669.01 &        vardepth &  2.4e-02 &  3.4e-04 &  5633 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.4 &  NaN \\
  6960913 &   59.9 &  151.2 &  K01361.01 &          planet &  3.5e-02 &  2.2e-03 &  4338 &     27 &   4.7 &  1.3e-02 &    0.6 &  2.1e-02 &   SM &    2.1 &  0.2 \\
  6964159 &   25.5 &  139.4 &  K03129.01 &  offset-no-star &  1.3e-02 &  1.2e-03 &  5806 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  7019524 &    5.3 &  134.3 &  K02877.01 &          planet &  1.0e-02 &  1.1e-03 &  5883 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.0 &  NaN \\
  7046804 &   11.7 &  142.2 &  K00205.01 &          planet &  9.3e-02 &  9.7e-04 &  5210 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    7.8 &  NaN \\
  7047207 &   19.1 &  138.4 &  K02494.01 &          planet &  1.4e-02 &  6.7e-04 &  5999 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.5 &  NaN \\
  7047299 &   35.9 &  165.6 &        NaN &          Vshape &  4.4e-01 &  2.5e-02 &  5885 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   42.8 &  NaN \\
  7090524 &    6.7 &  132.3 &  K02920.01 &          planet &  1.1e-02 &  1.2e-03 &  5707 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.1 &  NaN \\
  7091432 &   11.6 &  134.1 &        NaN &          planet &  1.7e-02 &  1.9e-03 &  5140 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.4 &  NaN \\
  7098355 &   29.0 &  141.6 &  K00454.01 &          planet &  2.8e-02 &  4.0e-03 &  5258 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.3 &  NaN \\
  7101828 &   47.9 &  145.3 &  K00455.01 &        vardepth &  2.2e-02 &  1.0e-03 &  4257 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.3 &  NaN \\
  7103919 &   10.8 &  140.3 &        NaN &          planet &  1.3e-02 &  9.7e-04 &  5483 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.3 &  NaN \\
  7105574 &   20.7 &  143.2 &        NaN &         eclipse &  5.0e-01 &  2.5e-03 &  6031 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   51.3 &  NaN \\
  7107802 &   10.4 &  137.5 &  K02420.01 &          planet &  1.4e-02 &  1.4e-03 &  5813 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  7115785 &   41.7 &  153.8 &  K00672.02 &          planet &  2.9e-02 &  4.2e-04 &  5543 &     97 &   4.5 &  2.9e-02 &    0.9 &  4.3e-02 &   SM &    2.9 &  0.1 \\
  7124026 &   15.7 &  145.6 &        NaN &          planet &  1.1e-02 &  3.2e-04 &  6088 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.2 &  NaN \\
  7133294 &   13.6 &  132.2 &        NaN &          planet &  8.3e-03 &  7.7e-04 &  5791 &    -99 &   4.1 &      NaN &    1.4 &      NaN &    P &    1.3 &  NaN \\
  7211221 &    5.6 &  136.9 &  K01379.01 &          planet &  1.2e-02 &  8.8e-04 &  5634 &     71 &   4.4 &  3.6e-02 &    0.9 &  4.6e-02 &   SM &    1.2 &  0.1 \\
  7219906 &   35.1 &  153.4 &        NaN &         eclipse &  1.1e-01 &  4.5e-03 &  5556 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    9.9 &  NaN \\
  7269974 &   13.7 &  144.1 &  K00456.01 &          planet &  3.2e-02 &  5.4e-04 &  5889 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.2 &  NaN \\
  7286173 &   56.4 &  151.4 &  K01862.01 &          planet &  2.3e-02 &  1.6e-03 &  5537 &     87 &   4.4 &  7.4e-02 &    1.1 &  1.0e-01 &   SM &    2.7 &  0.3 \\
  7286911 &   11.6 &  138.2 &  K02180.01 &          planet &  2.0e-02 &  1.2e-03 &  5630 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.8 &  NaN \\
  7289317 &   16.8 &  140.5 &  K02450.01 &          planet &  1.8e-02 &  1.9e-03 &  5784 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.8 &  NaN \\
  7289577 &  109.4 &  198.0 &  K01974.01 &          planet &  3.4e-02 &  7.8e-03 &  5403 &     44 &   4.5 &  4.7e-02 &    0.9 &  4.4e-02 &   SM &    3.2 &  0.8 \\
  7336754 &   12.2 &  133.8 &        NaN &         eclipse &  4.1e-01 &  1.7e-02 &  5798 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   44.8 &  NaN \\
  7353970 &  198.4 &  155.6 &        NaN &          Vshape &  3.1e-01 &  4.1e-03 &  5421 &     34 &   4.5 &  2.1e-02 &    0.9 &  3.3e-02 &   SM &   30.3 &  1.2 \\
  7357531 &  251.1 &  230.0 &  K01368.01 &          Vshape &  1.2e-01 &  1.7e-02 &  5710 &     60 &   4.3 &  8.1e-02 &    1.2 &  1.5e-01 &   SM &   15.0 &  2.9 \\
  7368664 &   12.9 &  144.3 &  K00614.01 &          planet &  7.0e-02 &  7.0e-03 &  5889 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    6.9 &  NaN \\
  7376490 &    5.9 &  136.4 &        NaN &         eclipse &  1.9e-01 &  1.1e-03 &  5802 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &   23.4 &  NaN \\
  7382313 &    7.4 &  133.1 &  K02392.01 &          planet &  1.3e-02 &  8.8e-04 &  5810 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.4 &  NaN \\
  7386827 &   10.4 &  137.7 &  K01704.01 &          planet &  2.4e-02 &  9.4e-04 &  5637 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.7 &  NaN \\
  7428316 &    7.1 &  137.5 &  K02809.01 &     offset-star &  1.3e-02 &  1.5e-03 &  6077 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.4 &  NaN \\
  7445445 &   10.7 &  137.9 &  K00567.01 &          planet &  2.5e-02 &  9.1e-04 &  5817 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.4 &  NaN \\
  7446631 &   29.2 &  144.0 &  K02598.01 &          planet &  1.2e-02 &  8.3e-04 &  6018 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.4 &  NaN \\
  7447200 &    8.0 &  131.7 &  K00676.01 &          planet &  5.1e-02 &  2.3e-04 &  4448 &     73 &   4.7 &  2.1e-02 &    0.6 &  2.8e-02 &   SM &    3.4 &  0.2 \\
  7455981 &   14.5 &  135.5 &        NaN &          planet &  7.9e-03 &  3.6e-04 &  5642 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    0.8 &  NaN \\
  7456001 &   40.1 &  151.8 &  K01517.01 &          planet &  2.9e-02 &  1.2e-03 &  6062 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    3.2 &  NaN \\
  7504328 &   53.7 &  154.4 &  K00458.01 &          planet &  6.3e-02 &  1.1e-02 &  5832 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &    8.1 &  NaN \\
  7534267 &   39.4 &  169.2 &  K03147.01 &          planet &  1.5e-02 &  1.1e-03 &  5764 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &    1.5 &  NaN \\
  7602070 &   11.8 &  140.8 &  K00514.01 &         eclipse &  2.2e-02 &  5.2e-04 &  5656 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.0 &  NaN \\
  7624297 &   18.0 &  148.7 &        NaN &         eclipse &  5.8e-01 &  5.5e-03 &  5366 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   47.8 &  NaN \\
  7626506 &    8.4 &  134.0 &  K00150.01 &          planet &  2.8e-02 &  6.4e-04 &  5535 &    155 &   4.4 &  5.7e-02 &    1.0 &  7.0e-02 &   SM &    2.9 &  0.2 \\
  7630229 &  278.1 &  177.5 &  K00683.01 &          planet &  5.0e-02 &  4.3e-03 &  5834 &     41 &   4.4 &  1.5e-02 &    1.0 &  2.6e-02 &   SM &    5.7 &  0.5 \\
  7668663 &    6.5 &  136.0 &  K01898.01 &          planet &  1.3e-02 &  7.1e-04 &  5726 &    151 &   4.3 &  1.5e-01 &    1.1 &  2.1e-01 &   SM &    1.6 &  0.3 \\
  7700622 &   35.6 &  153.5 &  K00315.01 &          planet &  2.7e-02 &  8.2e-04 &  4780 &     70 &   4.6 &  1.5e-02 &    0.7 &  1.9e-02 &   SM &    2.0 &  0.1 \\
  7742408 &   33.5 &  163.8 &        NaN &          planet &  1.1e-02 &  4.7e-04 &  4802 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    0.8 &  NaN \\
  7743464 &   55.2 &  165.0 &        NaN &          Vshape &  6.2e-01 &  2.7e-02 &  6013 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   63.4 &  NaN \\
  7747425 &    8.0 &  135.3 &  K01952.01 &          planet &  1.5e-02 &  6.8e-04 &  5998 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.7 &  NaN \\
  7750419 &   32.8 &  151.5 &  K01708.01 &          planet &  2.3e-02 &  2.2e-03 &  5890 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.2 &  NaN \\
  7768451 &  192.7 &  162.9 &  K01527.01 &          planet &  3.2e-02 &  3.0e-03 &  5405 &     77 &   4.5 &  3.3e-02 &    0.9 &  2.7e-02 &   SM &    3.1 &  0.3 \\
  7779077 &   16.8 &  138.0 &  K01842.01 &          planet &  2.6e-02 &  7.3e-04 &  5526 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.7 &  NaN \\
  7802136 &   11.0 &  137.2 &  K01449.01 &         eclipse &  2.2e-01 &  1.2e-03 &  6010 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   23.7 &  NaN \\
  7812179 &   17.8 &  134.0 &  K00515.01 &         eclipse &  3.4e-02 &  2.4e-03 &  5467 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.9 &  NaN \\
  7813039 &  141.7 &  167.4 &        NaN &          Vshape &  4.0e-02 &  7.4e-03 &  5611 &     56 &   4.5 &  4.0e-02 &    0.9 &  4.8e-02 &   SM &    4.1 &  0.8 \\
  7826659 &  211.0 &  279.1 &  K02686.01 &          planet &  4.1e-02 &  2.1e-03 &  4662 &     26 &   4.6 &  1.3e-02 &    0.7 &  1.4e-02 &   SM &    3.0 &  0.2 \\
  7830637 &  121.6 &  211.5 &  K01454.01 &          radius &  2.1e-01 &  1.8e-03 &  6076 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   22.2 &  NaN \\
  7833305 &    8.3 &  139.7 &        NaN &          planet &  7.9e-03 &  8.8e-04 &  5437 &    -99 &   4.0 &      NaN &    1.5 &      NaN &    P &    1.3 &  NaN \\
  7840044 &   13.5 &  144.0 &  K00516.01 &        vardepth &  1.5e-02 &  2.4e-03 &  5891 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.6 &  NaN \\
  7841925 &   14.2 &  140.6 &  K01499.01 &          planet &  2.6e-02 &  1.2e-03 &  5437 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    2.6 &  NaN \\
  7866914 &  366.0 &  182.7 &        NaN &         eclipse &  4.0e-02 &  1.1e-02 &  6082 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    4.4 &  NaN \\
  7870032 &   16.9 &  138.6 &  K01818.01 &          planet &  2.8e-02 &  1.6e-03 &  5497 &     91 &   4.5 &  3.8e-02 &    0.9 &  4.3e-02 &   SM &    2.6 &  0.2 \\
  7877978 &   56.6 &  146.6 &  K02760.01 &          planet &  2.5e-02 &  3.5e-03 &  4588 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.7 &  NaN \\
  7906671 &   45.1 &  157.0 &  K03018.01 &        vardepth &  1.7e-02 &  1.2e-03 &  5559 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.9 &  NaN \\
  7906739 &    7.0 &  136.9 &        NaN &        vardepth &  9.1e-03 &  4.0e-04 &  5951 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    0.9 &  NaN \\
  7906882 &   52.5 &  171.7 &  K00686.01 &          planet &  1.2e-01 &  1.4e-03 &  5589 &     90 &   4.4 &  6.1e-02 &    1.0 &  8.3e-02 &   SM &   12.9 &  1.1 \\
  7918652 &   11.5 &  136.3 &  K02984.01 &          planet &  7.9e-03 &  7.6e-04 &  6116 &     46 &   4.4 &  3.1e-02 &    1.1 &  4.7e-02 &   SM &    1.0 &  0.1 \\
  7938499 &   14.5 &  143.4 &        NaN &          planet &  1.2e-02 &  4.0e-04 &  4387 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    0.7 &  NaN \\
  7941200 &   65.7 &  137.4 &  K00092.01 &          planet &  2.5e-02 &  1.4e-03 &  5800 &     78 &   4.3 &  1.5e-01 &    1.2 &  2.3e-01 &   SM &    3.3 &  0.6 \\
  7949593 &   17.8 &  146.6 &        NaN &          planet &  1.1e-02 &  8.8e-04 &  6027 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    1.3 &  NaN \\
  7971389 &   13.2 &  136.5 &        NaN &          Vshape &  3.9e-01 &  8.9e-03 &  6077 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   44.0 &  NaN \\
  7975727 &   22.4 &  150.4 &  K00418.01 &         eclipse &  1.0e-01 &  1.3e-03 &  5352 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    9.8 &  NaN \\
  7977197 &   19.4 &  150.7 &  K00459.01 &          planet &  3.3e-02 &  3.2e-03 &  5833 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    3.5 &  NaN \\
  7987749 &   17.0 &  145.5 &        NaN &         eclipse &  4.1e-01 &  4.5e-03 &  5574 &    -99 &   4.1 &      NaN &    1.4 &      NaN &    P &   61.0 &  NaN \\
  7989422 &    7.5 &  133.4 &  K02151.01 &        vardepth &  9.0e-03 &  5.2e-04 &  6012 &    -99 &   4.2 &      NaN &    1.4 &      NaN &    P &    1.3 &  NaN \\
  8008067 &   15.8 &  137.6 &        NaN &          planet &  2.1e-02 &  7.1e-04 &  5594 &     88 &   4.4 &  3.0e-02 &    1.1 &  2.5e-02 &   SM &    2.5 &  0.1 \\
  8008206 &   20.7 &  144.0 &  K00569.01 &          planet &  2.5e-02 &  2.4e-03 &  5174 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
  8009496 &   38.5 &  150.6 &        NaN &        vardepth &  2.1e-02 &  5.9e-04 &  6097 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.2 &  NaN \\
  8009500 &   38.5 &  150.6 &        NaN &         eclipse &  3.9e-01 &  9.4e-04 &  5329 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   35.6 &  NaN \\
  8017703 &   14.0 &  140.0 &  K00518.01 &          planet &  2.9e-02 &  4.3e-04 &  4917 &     81 &   4.6 &  2.0e-02 &    0.7 &  1.7e-02 &   SM &    2.2 &  0.1 \\
  8022244 &   11.9 &  142.6 &  K00519.01 &          planet &  2.5e-02 &  1.3e-03 &  6027 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.6 &  NaN \\
  8022489 &  197.5 &  272.4 &  K02674.01 &          planet &  5.3e-02 &  8.9e-04 &  5756 &    156 &   4.2 &  2.8e-01 &    1.5 &  6.5e-01 &   SM &    8.8 &  3.7 \\
  8023317 &   16.6 &  146.7 &        NaN &         eclipse &  2.0e-01 &  2.9e-03 &  5862 &    -99 &   4.1 &      NaN &    1.6 &      NaN &    P &   34.9 &  NaN \\
  8041216 &    8.5 &  134.8 &  K00237.01 &          planet &  2.3e-02 &  8.3e-04 &  5767 &    108 &   4.4 &  5.2e-02 &    1.1 &  8.0e-02 &   SM &    2.7 &  0.2 \\
  8043638 &   17.6 &  140.9 &  K00460.01 &          planet &  3.4e-02 &  5.8e-04 &  5520 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    3.7 &  NaN \\
  8044608 &  106.2 &  234.6 &        NaN &         eclipse &  5.5e-01 &  2.8e-02 &  6095 &    -99 &   4.3 &      NaN &    1.3 &      NaN &    P &   76.6 &  NaN \\
  8074805 &  170.9 &  186.0 &  K02670.01 &          planet &  3.7e-02 &  3.5e-03 &  5987 &    107 &   4.2 &  1.4e-01 &    1.4 &  2.2e-01 &   SM &    5.7 &  1.0 \\
  8087812 &   27.2 &  132.4 &        NaN &          planet &  9.8e-03 &  9.0e-04 &  6014 &    -99 &   4.2 &      NaN &    1.4 &      NaN &    P &    1.5 &  NaN \\
  8095441 &   11.9 &  140.2 &  K02743.01 &          planet &  1.4e-02 &  1.4e-03 &  5530 &     69 &   4.5 &  2.8e-02 &    0.9 &  3.6e-02 &   SM &    1.3 &  0.1 \\
  8099138 &   66.2 &  141.6 &  K02338.01 &          planet &  2.1e-02 &  2.4e-03 &  5899 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.1 &  NaN \\
  8107225 &    5.6 &  133.8 &  K00235.01 &          planet &  2.3e-02 &  7.8e-04 &  5127 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.8 &  NaN \\
  8107380 &   14.0 &  142.2 &  K00162.01 &          planet &  2.4e-02 &  3.0e-04 &  5795 &     73 &   4.3 &  7.1e-02 &    1.2 &  1.0e-01 &   SM &    3.1 &  0.3 \\
  8121328 &   19.1 &  145.6 &        NaN &          planet &  1.2e-02 &  7.6e-04 &  5430 &    -99 &   4.0 &      NaN &    1.5 &      NaN &    P &    2.0 &  NaN \\
  8127586 &   16.6 &  147.6 &        NaN &  offset-no-star &  1.8e-02 &  7.9e-04 &  6043 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.0 &  NaN \\
  8127607 &   16.6 &  147.6 &        NaN &        vardepth &  2.2e-02 &  2.3e-03 &  5225 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.8 &  NaN \\
  8142787 &  178.1 &  210.1 &        NaN &          planet &  2.6e-02 &  2.4e-03 &  5431 &     65 &   4.5 &  2.9e-02 &    0.9 &  2.3e-02 &   SM &    2.5 &  0.2 \\
  8142942 &    5.8 &  133.9 &  K01985.01 &          planet &  2.8e-02 &  2.4e-03 &  4931 &     64 &   4.6 &  3.8e-03 &    0.7 &  1.3e-02 &   SM &    2.2 &  0.2 \\
  8160953 &  116.3 &  173.7 &  K01858.01 &          planet &  3.9e-02 &  1.5e-03 &  5354 &     61 &   4.5 &  3.7e-02 &    0.8 &  3.7e-02 &   SM &    3.5 &  0.2 \\
  8168187 &   18.3 &  142.9 &  K02209.01 &          planet &  1.4e-02 &  1.4e-03 &  5744 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.4 &  NaN \\
  8183288 &   66.6 &  171.2 &        NaN &          planet &  2.1e-02 &  1.3e-03 &  4550 &     72 &   4.7 &  1.7e-02 &    0.6 &  2.3e-02 &   SM &    1.4 &  0.1 \\
  8193178 &   10.6 &  137.2 &  K00572.01 &          planet &  2.1e-02 &  9.0e-04 &  6166 &     62 &   4.4 &  3.1e-02 &    1.1 &  5.7e-02 &   SM &    2.6 &  0.2 \\
  8197343 &   11.8 &  134.6 &  K01746.01 &          planet &  1.9e-02 &  1.4e-03 &  5965 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.9 &  NaN \\
  8210721 &   22.7 &  138.2 &        NaN &         eclipse &  2.4e-01 &  2.3e-03 &  5584 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &   27.4 &  NaN \\
  8218379 &   16.6 &  133.9 &  K01920.01 &          planet &  2.4e-02 &  6.7e-04 &  5488 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.0 &  NaN \\
  8219673 &   20.1 &  149.1 &  K00419.01 &          planet &  1.5e-01 &  3.5e-03 &  5986 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   14.8 &  NaN \\
  8223328 &   35.5 &  165.9 &        NaN &          planet &  1.1e-01 &  1.7e-03 &  5719 &    -99 &   4.2 &      NaN &    1.3 &      NaN &    P &   16.7 &  NaN \\
  8226050 &   34.3 &  147.0 &  K01910.01 &          planet &  2.4e-02 &  9.5e-04 &  5299 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.2 &  NaN \\
  8233802 &   69.4 &  154.2 &        NaN &        vardepth &  2.3e-02 &  2.6e-03 &  5803 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.2 &  NaN \\
  8242434 &   45.0 &  144.6 &  K01726.01 &          planet &  2.6e-02 &  6.5e-04 &  4684 &     34 &   4.6 &  1.2e-02 &    0.7 &  1.6e-02 &   SM &    1.9 &  0.1 \\
  8247770 &    8.3 &  136.3 &  K02569.01 &          planet &  1.0e-02 &  1.2e-03 &  5650 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.2 &  NaN \\
  8260234 &    5.7 &  132.1 &        NaN &          planet &  1.5e-02 &  6.7e-04 &  5237 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.3 &  NaN \\
  8260902 &   38.7 &  157.6 &  K02144.01 &          planet &  2.2e-02 &  7.7e-04 &  5420 &    -99 &   4.0 &      NaN &    1.5 &      NaN &    P &    3.7 &  NaN \\
  8265218 &   12.8 &  144.3 &  K00522.01 &          planet &  3.3e-02 &  2.2e-03 &  5897 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.3 &  NaN \\
  8280511 &   10.4 &  134.8 &        NaN &          planet &  1.6e-02 &  1.1e-03 &  5489 &     86 &   4.5 &  5.5e-02 &    0.9 &  6.5e-02 &   SM &    1.6 &  0.2 \\
  8301878 &   20.7 &  140.9 &        NaN &          planet &  1.2e-02 &  1.2e-03 &  5613 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.2 &  NaN \\
  8313667 &   30.6 &  132.3 &  K01145.01 &          planet &  1.9e-02 &  5.4e-04 &  5943 &    136 &   4.4 &  3.3e-02 &    1.1 &  1.6e-02 &   SM &    2.3 &  0.1 \\
  8321314 &   15.0 &  145.0 &  K02293.01 &          planet &  1.7e-02 &  1.4e-03 &  5451 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.8 &  NaN \\
  8323753 &    6.7 &  134.3 &  K00175.01 &        vardepth &  1.9e-02 &  6.0e-04 &  6075 &    -99 &   4.3 &      NaN &    1.3 &      NaN &    P &    2.6 &  NaN \\
  8326342 &   14.4 &  142.0 &  K02680.01 &          planet &  5.1e-02 &  1.2e-02 &  5474 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    4.4 &  NaN \\
  8332986 &  302.4 &  309.2 &        NaN &          Vshape &  1.6e-01 &  3.6e-02 &  5330 &     18 &   4.5 &  3.9e-02 &    0.8 &  4.3e-02 &   SM &   14.3 &  3.4 \\
  8344004 &    6.0 &  136.5 &  K00573.01 &          planet &  2.4e-02 &  6.8e-04 &  6010 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    3.0 &  NaN \\
  8349399 &   56.4 &  170.6 &        NaN &          planet &  1.0e-02 &  1.3e-03 &  5980 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    1.3 &  NaN \\
  8349582 &   11.5 &  132.0 &  K00122.01 &          planet &  2.3e-02 &  6.2e-04 &  5695 &     46 &   4.3 &  1.1e-01 &    1.3 &  1.9e-01 &   SM &    3.2 &  0.5 \\
  8352537 &    6.0 &  132.0 &  K00420.01 &          planet &  5.3e-02 &  1.8e-03 &  4860 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    4.0 &  NaN \\
  8355239 &   20.1 &  151.2 &  K00574.01 &          planet &  3.0e-02 &  1.3e-03 &  5217 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.3 &  NaN \\
  8358008 &   10.1 &  135.3 &        NaN &         eclipse &  1.6e-01 &  6.4e-04 &  5260 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   14.7 &  NaN \\
  8358012 &   10.1 &  135.3 &  K02929.01 &          planet &  1.7e-02 &  2.0e-03 &  5387 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.4 &  NaN \\
  8364115 &    7.7 &  138.0 &        NaN &         eclipse &  2.0e-02 &  2.1e-04 &  5953 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.1 &  NaN \\
  8364119 &    7.7 &  138.0 &        NaN &         eclipse &  7.5e-01 &  3.5e-02 &  5661 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   68.4 &  NaN \\
  8374580 &  176.2 &  192.5 &  K00615.01 &          Vshape &  1.0e-01 &  1.3e-02 &  5565 &     89 &   4.2 &  1.6e-01 &    1.4 &  2.9e-01 &   SM &   15.5 &  3.8 \\
  8378922 &   43.3 &  150.4 &        NaN &          Vshape &  7.9e-01 &  2.2e-02 &  5676 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   89.1 &  NaN \\
  8409295 &   82.3 &  212.0 &        NaN &          planet &  1.8e-02 &  3.2e-03 &  6049 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.9 &  NaN \\
  8429668 &    5.0 &  134.7 &        NaN &     offset-star &  7.6e-03 &  8.4e-04 &  5306 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    0.6 &  NaN \\
  8453211 &    5.8 &  131.5 &  K00236.01 &        vardepth &  2.8e-02 &  1.4e-02 &  5578 &    -99 &   4.3 &      NaN &    1.0 &      NaN &    P &    3.2 &  NaN \\
  8460600 &    6.4 &  134.2 &        NaN &         eclipse &  2.4e-01 &  1.1e-03 &  5163 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   19.9 &  NaN \\
  8474898 &  199.4 &  240.9 &  K00576.01 &          Vshape &  8.8e-02 &  1.2e-02 &  5650 &     96 &   4.3 &  1.7e-01 &    1.3 &  2.7e-01 &   SM &   12.1 &  3.1 \\
  8481129 &   16.3 &  133.8 &  K02402.01 &          planet &  1.5e-02 &  9.9e-04 &  4763 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.1 &  NaN \\
  8491277 &    9.6 &  132.2 &  K00234.01 &          planet &  2.6e-02 &  9.0e-04 &  5940 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    3.1 &  NaN \\
  8509781 &   70.3 &  199.0 &        NaN &          radius &  2.1e-01 &  2.2e-02 &  6074 &    -99 &   4.2 &      NaN &    1.4 &      NaN &    P &   31.6 &  NaN \\
  8543278 &    7.5 &  135.0 &        NaN &         eclipse &  2.4e-01 &  1.9e-02 &  5159 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   18.5 &  NaN \\
  8547429 &   11.7 &  140.6 &  K02658.01 &          planet &  1.2e-02 &  8.6e-04 &  6009 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.2 &  NaN \\
  8552719 &   88.4 &  176.3 &        NaN &          planet &  3.8e-02 &  8.4e-04 &  5288 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    3.2 &  NaN \\
  8559863 &   22.5 &  143.3 &        NaN &         eclipse &  3.3e-01 &  1.3e-03 &  5375 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   27.0 &  NaN \\
  8560940 &   32.0 &  133.9 &        NaN &          planet &  1.0e-02 &  7.8e-04 &  5852 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.0 &  NaN \\
  8564587 &    5.7 &  132.8 &  K01270.01 &          planet &  2.7e-02 &  1.3e-03 &  5289 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.1 &  NaN \\
  8564674 &    5.9 &  135.5 &  K02022.01 &          planet &  1.8e-02 &  4.4e-04 &  5936 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.8 &  NaN \\
  8565266 &    6.4 &  137.8 &  K00578.01 &          planet &  3.1e-02 &  5.5e-04 &  5990 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    3.7 &  NaN \\
  8572936 &   27.8 &  146.7 &        NaN &          radius &  8.4e-01 &  8.9e-03 &  6003 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   92.5 &  NaN \\
  8573193 &    8.2 &  134.6 &        NaN &          planet &  1.0e-02 &  1.1e-03 &  5981 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.0 &  NaN \\
  8580438 &    6.5 &  135.5 &        NaN &         eclipse &  3.0e-01 &  1.9e-04 &  5504 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   31.3 &  NaN \\
  8583696 &   50.3 &  167.7 &  K01275.01 &          planet &  3.4e-02 &  1.6e-03 &  5907 &    140 &   4.3 &  1.5e-01 &    1.2 &  2.2e-01 &   SM &    4.5 &  0.8 \\
  8591693 &   29.5 &  154.2 &  K02123.01 &          planet &  2.2e-02 &  1.8e-03 &  6030 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.2 &  NaN \\
  8611257 &   99.3 &  148.6 &  K02931.01 &          planet &  2.1e-02 &  3.2e-03 &  4995 &     37 &   4.6 &  5.6e-03 &    0.7 &  1.6e-02 &   SM &    1.7 &  0.3 \\
  8611781 &   77.0 &  192.3 &  K02185.01 &          planet &  1.9e-02 &  2.1e-03 &  5887 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.2 &  NaN \\
  8611832 &   22.6 &  140.4 &  K02414.01 &          planet &  1.3e-02 &  8.5e-04 &  5587 &    151 &   4.4 &  3.3e-02 &    1.0 &  6.4e-02 &   SM &    1.4 &  0.1 \\
  8618226 &    5.9 &  131.8 &        NaN &         eclipse &  6.6e-01 &  3.0e-02 &  6044 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &   81.1 &  NaN \\
  8621348 &   11.3 &  138.8 &  K00461.01 &        vardepth &  2.1e-02 &  7.3e-04 &  5643 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.9 &  NaN \\
  8625732 &   32.0 &  133.9 &        NaN &          planet &  9.4e-03 &  7.1e-04 &  5597 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    0.8 &  NaN \\
  8625925 &    6.5 &  136.6 &  K00580.01 &          planet &  2.6e-02 &  1.9e-03 &  5795 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.5 &  NaN \\
  8628758 &   14.4 &  138.2 &  K01279.01 &          planet &  1.7e-02 &  3.6e-04 &  5771 &     34 &   4.4 &  4.6e-02 &    1.1 &  5.1e-02 &   SM &    1.9 &  0.1 \\
  8644288 &   14.9 &  143.0 &  K00137.02 &          planet &  5.2e-02 &  6.7e-04 &  5424 &     40 &   4.5 &  2.0e-02 &    0.9 &  3.4e-02 &   SM &    5.2 &  0.2 \\
  8644365 &   19.9 &  139.4 &        NaN &          planet &  1.1e-02 &  6.9e-04 &  6049 &     63 &   4.4 &  2.0e-02 &    1.1 &  3.9e-02 &   SM &    1.3 &  0.1 \\
  8644545 &  296.0 &  138.9 &        NaN &          planet &  1.9e-02 &  2.8e-03 &  5507 &     93 &   4.4 &  5.0e-02 &    1.0 &  6.3e-02 &   SM &    2.0 &  0.3 \\
  8652999 &   15.2 &  136.5 &        NaN &        vardepth &  1.7e-02 &  2.0e-03 &  5892 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &    2.2 &  NaN \\
  8681734 &    7.7 &  137.6 &  K02340.01 &          planet &  1.6e-02 &  9.8e-04 &  5621 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.7 &  NaN \\
  8686097 &  172.7 &  236.9 &  K00374.01 &          planet &  2.6e-02 &  1.7e-03 &  5706 &    146 &   4.3 &  2.8e-02 &    1.0 &  6.5e-02 &   SM &    3.0 &  0.3 \\
  8692861 &   13.7 &  137.8 &  K00172.01 &          planet &  2.2e-02 &  5.9e-04 &  5603 &    151 &   4.4 &  3.4e-02 &    1.0 &  6.3e-02 &   SM &    2.4 &  0.2 \\
  8733497 &   76.8 &  188.1 &        NaN &          radius &  5.7e-01 &  7.3e-02 &  5692 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   52.1 &  NaN \\
  8742590 &   49.5 &  141.8 &  K01281.01 &          planet &  2.2e-02 &  1.5e-03 &  5773 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.0 &  NaN \\
  8746295 &    6.9 &  136.0 &  K02475.01 &          planet &  1.4e-02 &  2.7e-03 &  5691 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  8751933 &   86.6 &  173.8 &  K01257.01 &          planet &  7.8e-02 &  2.2e-03 &  5472 &     74 &   4.4 &  6.6e-02 &    1.0 &  7.5e-02 &   SM &    8.4 &  0.7 \\
  8802165 &   17.4 &  132.0 &  K00694.01 &          planet &  2.8e-02 &  2.2e-04 &  5702 &     46 &   4.4 &  6.5e-02 &    1.1 &  8.6e-02 &   SM &    3.2 &  0.3 \\
  8804283 &   22.8 &  138.7 &  K01276.01 &          planet &  2.4e-02 &  1.9e-03 &  5594 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
  8804455 &    7.6 &  132.0 &  K02159.01 &          planet &  9.8e-03 &  4.5e-04 &  5714 &     92 &   4.4 &  4.7e-02 &    1.1 &  6.1e-02 &   SM &    1.1 &  0.1 \\
  8804845 &    5.4 &  135.9 &  K02039.01 &          planet &  1.6e-02 &  1.7e-03 &  5597 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.4 &  NaN \\
  8806072 &   40.1 &  169.9 &  K01273.01 &          planet &  3.3e-02 &  1.1e-03 &  5633 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    3.0 &  NaN \\
  8822216 &    7.0 &  133.9 &  K00581.01 &          planet &  3.3e-02 &  6.6e-04 &  5653 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    3.0 &  NaN \\
  8826168 &   11.6 &  134.9 &  K01850.01 &          planet &  1.9e-02 &  9.1e-04 &  5905 &    113 &   4.4 &  3.9e-02 &    1.1 &  4.4e-02 &   SM &    2.2 &  0.1 \\
  8827575 &   15.6 &  144.9 &  K03052.02 &          planet &  1.0e-02 &  5.4e-04 &  5386 &     90 &   4.5 &  2.3e-02 &    0.8 &  2.9e-02 &   SM &    0.9 &  0.1 \\
  8832512 &   10.0 &  131.8 &        NaN &          planet &  2.9e-02 &  1.3e-03 &  5487 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    3.0 &  NaN \\
  8848271 &   10.0 &  137.4 &  K01256.01 &         eclipse &  1.0e-01 &  8.0e-04 &  5855 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &   12.2 &  NaN \\
  8869680 &    7.0 &  132.0 &  K00696.01 &  offset-no-star &  1.2e-02 &  6.1e-04 &  5964 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    1.5 &  NaN \\
  8879427 &   16.3 &  136.9 &        NaN &         eclipse &  2.7e-01 &  1.9e-03 &  5995 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   29.5 &  NaN \\
  8890783 &   58.4 &  138.2 &  K00464.01 &          planet &  6.7e-02 &  1.3e-03 &  5490 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    6.6 &  NaN \\
  8939211 &   54.2 &  137.2 &        NaN &         eclipse &  1.3e-02 &  2.5e-04 &  5984 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.4 &  NaN \\
  8949247 &   23.8 &  152.6 &  K01387.01 &          radius &  2.5e-01 &  1.7e-03 &  5918 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   26.0 &  NaN \\
  8950568 &    8.3 &  139.7 &  K02038.01 &          planet &  1.8e-02 &  6.1e-04 &  5438 &     64 &   4.5 &  2.9e-02 &    0.9 &  2.0e-02 &   SM &    1.8 &  0.1 \\
  8962094 &   30.9 &  142.1 &  K00700.01 &          planet &  2.2e-02 &  1.1e-03 &  5785 &    162 &   4.3 &  2.9e-02 &    1.1 &  6.3e-02 &   SM &    2.5 &  0.2 \\
  8972058 &    9.0 &  136.7 &  K00159.01 &          planet &  2.1e-02 &  1.5e-03 &  5964 &    134 &   4.4 &  2.9e-02 &    1.1 &  2.1e-02 &   SM &    2.5 &  0.2 \\
  8973000 &   28.0 &  148.8 &        NaN &          radius &  4.1e-01 &  9.5e-04 &  5407 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   35.7 &  NaN \\
  8984706 &   10.1 &  137.5 &        NaN &         eclipse &  7.2e-01 &  7.6e-03 &  5914 &    -99 &   4.1 &      NaN &    1.5 &      NaN &    P &  117.2 &  NaN \\
  9002278 &   18.2 &  144.5 &  K00701.01 &          planet &  2.8e-02 &  6.2e-04 &  4966 &      9 &   4.6 &  6.2e-03 &    0.7 &  1.1e-02 &   SM &    2.1 &  0.1 \\
  9006186 &    5.5 &  134.1 &  K02169.01 &          planet &  9.0e-03 &  6.3e-04 &  5395 &     48 &   4.5 &  1.7e-02 &    0.9 &  2.3e-02 &   SM &    0.9 &  0.1 \\
  9006449 &   12.6 &  138.6 &  K01413.01 &          planet &  1.3e-02 &  3.2e-04 &  5630 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  9020160 &    5.9 &  134.8 &  K00582.01 &          planet &  2.7e-02 &  1.3e-03 &  5236 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.2 &  NaN \\
  9025971 &  141.2 &  256.2 &        NaN &          planet &  1.0e-01 &  1.0e-03 &  5710 &     48 &   4.4 &  6.9e-02 &    1.1 &  9.3e-02 &   SM &   12.1 &  1.1 \\
  9031703 &    9.3 &  137.6 &        NaN &          planet &  8.6e-03 &  5.2e-04 &  5490 &    -99 &   4.1 &      NaN &    1.5 &      NaN &    P &    1.4 &  NaN \\
  9042357 &   16.0 &  146.4 &        NaN &          planet &  2.3e-02 &  2.2e-03 &  5367 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.0 &  NaN \\
  9086154 &  225.3 &  225.0 &        NaN &          planet &  1.9e-02 &  1.9e-03 &  5795 &     64 &   4.3 &  9.2e-02 &    1.3 &  1.4e-01 &   SM &    2.7 &  0.4 \\
  9101496 &    6.6 &  132.6 &  K01915.01 &          planet &  1.5e-02 &  8.5e-04 &  5873 &    117 &   4.1 &  1.7e-01 &    1.7 &  3.8e-01 &   SM &    2.9 &  0.6 \\
  9116075 &   24.5 &  154.7 &        NaN &          planet &  1.3e-02 &  2.1e-03 &  4570 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    0.8 &  NaN \\
  9119458 &   11.5 &  139.1 &  K00525.01 &          planet &  2.8e-02 &  1.5e-03 &  5738 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    3.5 &  NaN \\
  9119568 &    5.5 &  134.0 &  K03087.01 &  offset-no-star &  7.9e-03 &  4.6e-04 &  5257 &     73 &   4.5 &  1.5e-02 &    0.9 &  2.4e-02 &   SM &    0.7 &  0.0 \\
  9139084 &    5.8 &  134.9 &  K00323.01 &          planet &  2.1e-02 &  4.6e-04 &  5403 &     68 &   4.5 &  4.1e-02 &    0.8 &  3.9e-02 &   SM &    1.9 &  0.1 \\
  9146018 &    9.9 &  136.0 &  K00584.01 &          planet &  2.8e-02 &  9.5e-04 &  5464 &     74 &   4.5 &  2.0e-02 &    0.9 &  2.2e-02 &   SM &    2.9 &  0.1 \\
  9150827 &   14.5 &  145.4 &  K01408.01 &          planet &  2.1e-02 &  1.0e-03 &  4252 &     69 &   4.7 &  1.0e-02 &    0.5 &  7.2e-02 &   SM &    1.1 &  0.2 \\
  9164836 &   48.1 &  170.8 &  K00213.01 &         eclipse &  3.9e-01 &  8.7e-03 &  6031 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   40.2 &  NaN \\
  9177629 &    5.6 &  133.8 &  K02522.01 &          planet &  1.2e-02 &  1.2e-03 &  4849 &     63 &   4.6 &  2.3e-02 &    0.8 &  3.3e-02 &   SM &    1.0 &  0.1 \\
  9226339 &   21.5 &  132.2 &        NaN &          planet &  1.0e-02 &  5.7e-04 &  5995 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &    1.4 &  NaN \\
  9266285 &    5.6 &  132.6 &        NaN &         eclipse &  3.7e-01 &  4.3e-04 &  4452 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &   23.7 &  NaN \\
  9266431 &   18.4 &  148.3 &  K00704.01 &          planet &  2.8e-02 &  1.5e-03 &  5313 &     73 &   4.6 &  9.1e-03 &    0.8 &  2.1e-02 &   SM &    2.4 &  0.1 \\
  9283156 &    5.2 &  132.8 &  K02657.01 &          planet &  6.4e-03 &  3.8e-04 &  5422 &     91 &   4.5 &  9.9e-03 &    0.8 &  2.4e-02 &   SM &    0.6 &  0.0 \\
  9284741 &   20.7 &  141.2 &        NaN &         eclipse &  7.9e-01 &  1.6e-02 &  5265 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   71.6 &  NaN \\
  9334893 &   16.7 &  141.8 &  K02298.01 &          planet &  1.2e-02 &  7.2e-04 &  4922 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    0.9 &  NaN \\
  9353182 &   10.5 &  136.5 &        NaN &         eclipse &  3.2e-01 &  5.5e-05 &  6100 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &   42.7 &  NaN \\
  9353314 &    5.2 &  131.9 &  K01900.01 &          planet &  2.0e-02 &  1.6e-03 &  4451 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.3 &  NaN \\
  9364290 &    5.3 &  136.4 &  K02374.01 &          planet &  1.3e-02 &  9.3e-04 &  5622 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.4 &  NaN \\
  9364609 &   15.0 &  141.5 &  K02137.01 &          planet &  1.6e-02 &  1.1e-03 &  5332 &     19 &   4.5 &  4.2e-02 &    0.8 &  3.4e-02 &   SM &    1.4 &  0.1 \\
  9394762 &   77.1 &  166.6 &        NaN &          planet &  2.2e-02 &  3.0e-03 &  5688 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.0 &  NaN \\
  9412445 &   10.2 &  132.6 &        NaN &  offset-no-star &  1.5e-02 &  3.4e-04 &  4168 &    -99 &   4.7 &      NaN &    0.5 &      NaN &    P &    0.9 &  NaN \\
  9412462 &   10.2 &  132.5 &        NaN &         eclipse &  7.8e-01 &  7.7e-03 &  5540 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   77.0 &  NaN \\
  9412760 &    9.4 &  137.4 &  K01977.01 &          planet &  2.0e-02 &  1.8e-03 &  4346 &    344 &   4.7 &  1.4e-01 &    0.6 &  9.8e-02 &   SM &    1.3 &  0.2 \\
  9425139 &  305.1 &  294.1 &        NaN &          planet &  5.9e-02 &  3.3e-03 &  5642 &     56 &   4.4 &  3.9e-02 &    1.1 &  4.3e-02 &   SM &    7.2 &  0.5 \\
  9447166 &   62.9 &  166.0 &        NaN &          planet &  1.9e-02 &  2.6e-03 &  4838 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.4 &  NaN \\
  9455325 &    9.8 &  139.5 &  K01813.01 &          planet &  2.2e-02 &  5.6e-04 &  5369 &     65 &   4.5 &  4.6e-02 &    0.9 &  4.5e-02 &   SM &    2.0 &  0.1 \\
  9458343 &   11.9 &  132.9 &  K02246.01 &          planet &  1.3e-02 &  1.2e-03 &  5650 &    106 &   4.4 &  5.6e-02 &    1.0 &  6.1e-02 &   SM &    1.4 &  0.2 \\
  9471974 &   49.2 &  141.9 &  K00119.01 &          planet &  3.8e-02 &  6.3e-04 &  5642 &     83 &   4.2 &  1.5e-01 &    1.4 &  2.3e-01 &   SM &    5.9 &  1.0 \\
  9472000 &   31.6 &  155.6 &  K02082.01 &          planet &  1.7e-02 &  9.6e-04 &  5875 &     84 &   4.2 &  1.4e-01 &    1.5 &  2.8e-01 &   SM &    2.8 &  0.5 \\
  9489953 &   58.3 &  169.8 &        NaN &          planet &  3.4e-02 &  1.4e-02 &  5861 &    -99 &   4.2 &      NaN &    1.3 &      NaN &    P &    4.9 &  NaN \\
  9491832 &   49.6 &  170.7 &        NaN &          planet &  1.0e-02 &  5.3e-04 &  5641 &    -99 &   4.1 &      NaN &    1.5 &      NaN &    P &    1.7 &  NaN \\
  9509343 &    6.4 &  135.6 &        NaN &          planet &  1.3e-02 &  1.2e-03 &  5390 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
  9514372 &  145.8 &  215.0 &        NaN &          planet &  2.1e-02 &  2.9e-03 &  5574 &     56 &   4.4 &  4.2e-02 &    0.9 &  4.1e-02 &   SM &    2.1 &  0.3 \\
  9520838 &  105.3 &  207.2 &  K01866.01 &          planet &  3.4e-02 &  2.6e-03 &  5530 &     77 &   4.5 &  2.6e-02 &    0.9 &  3.3e-02 &   SM &    3.3 &  0.3 \\
  9527915 &   13.2 &  139.6 &  K00165.01 &          planet &  2.7e-02 &  5.7e-04 &  5214 &     75 &   4.6 &  1.9e-02 &    0.8 &  1.8e-02 &   SM &    2.3 &  0.1 \\
  9549471 &   15.7 &  132.1 &        NaN &         eclipse &  8.9e-02 &  7.9e-03 &  5818 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    9.4 &  NaN \\
  9549472 &   15.7 &  132.1 &        NaN &         eclipse &  2.9e-01 &  4.0e-03 &  5842 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   31.9 &  NaN \\
  9570741 &   15.8 &  144.4 &  K00586.01 &          planet &  2.3e-02 &  1.2e-03 &  5934 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.2 &  NaN \\
  9571186 &   35.0 &  163.5 &        NaN &          planet &  2.2e-02 &  1.7e-03 &  4805 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.6 &  NaN \\
  9573539 &   10.0 &  139.1 &  K00180.01 &          planet &  2.4e-02 &  1.6e-03 &  5566 &     54 &   4.5 &  5.5e-02 &    0.9 &  6.6e-02 &   SM &    2.5 &  0.2 \\
  9576197 &    8.0 &  136.2 &        NaN &         eclipse &  2.4e-01 &  2.0e-04 &  5311 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   20.6 &  NaN \\
  9578686 &   21.4 &  136.0 &  K00709.01 &          planet &  2.4e-02 &  1.0e-03 &  5343 &     29 &   4.5 &  4.0e-02 &    0.9 &  4.2e-02 &   SM &    2.3 &  0.1 \\
  9583881 &   18.0 &  146.4 &  K00467.01 &          planet &  5.2e-02 &  1.4e-03 &  5803 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    5.0 &  NaN \\
  9589524 &   22.2 &  152.4 &  K00468.01 &          planet &  4.4e-02 &  1.1e-03 &  5132 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    3.7 &  NaN \\
  9597058 &   12.1 &  135.4 &  K01819.01 &          planet &  2.1e-02 &  6.2e-04 &  5368 &     66 &   4.5 &  3.8e-02 &    0.8 &  4.3e-02 &   SM &    1.9 &  0.1 \\
  9597345 &   44.7 &  174.8 &  K00711.01 &          planet &  2.6e-02 &  3.6e-04 &  5556 &     67 &   4.4 &  8.4e-02 &    1.1 &  1.1e-01 &   SM &    3.1 &  0.3 \\
  9607164 &   14.0 &  143.5 &  K00587.01 &          planet &  2.6e-02 &  9.8e-04 &  5290 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.4 &  NaN \\
  9631762 &   10.4 &  134.3 &  K00588.01 &          planet &  2.5e-02 &  1.6e-03 &  4678 &    -99 &   4.6 &      NaN &    0.6 &      NaN &    P &    1.7 &  NaN \\
  9631995 &    7.9 &  137.8 &  K00022.01 &          planet &  9.1e-02 &  7.3e-05 &  5834 &     71 &   4.3 &  7.9e-02 &    1.3 &  1.3e-01 &   SM &   12.6 &  1.3 \\
  9632895 &   27.3 &  132.4 &  K01451.01 &         eclipse &  2.5e-01 &  7.5e-05 &  5662 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   23.0 &  NaN \\
  9635606 &   48.9 &  153.8 &  K02535.01 &          planet &  2.0e-02 &  1.1e-03 &  4930 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.5 &  NaN \\
  9636569 &   10.6 &  139.8 &  K00527.01 &        vardepth &  1.5e-02 &  8.7e-04 &  5897 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.5 &  NaN \\
  9651234 &   96.9 &  187.1 &  K01938.01 &          planet &  2.8e-02 &  2.2e-03 &  5170 &     58 &   4.6 &  2.3e-02 &    0.8 &  1.5e-02 &   SM &    2.3 &  0.2 \\
  9661979 &   69.9 &  160.7 &  K02132.01 &          planet &  2.2e-02 &  2.3e-03 &  5584 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
  9662811 &   43.0 &  137.7 &  K01854.01 &          planet &  2.1e-02 &  8.6e-04 &  5548 &     54 &   4.5 &  6.2e-02 &    0.9 &  7.1e-02 &   SM &    2.1 &  0.2 \\
  9663113 &   20.7 &  142.8 &  K00179.01 &          planet &  2.9e-02 &  3.1e-04 &  6230 &    162 &   4.3 &  7.6e-02 &    1.4 &  1.3e-01 &   SM &    4.4 &  0.4 \\
  9673173 &   21.3 &  147.1 &        NaN &         eclipse &  5.0e-01 &  3.2e-03 &  6024 &    -99 &   4.2 &      NaN &    1.3 &      NaN &    P &   69.9 &  NaN \\
  9704384 &    5.5 &  132.3 &  K01913.01 &          planet &  1.3e-02 &  7.0e-04 &  5448 &     56 &   4.5 &  3.1e-02 &    0.9 &  3.8e-02 &   SM &    1.3 &  0.1 \\
  9714358 &    6.5 &  134.4 &        NaN &         eclipse &  4.5e-01 &  3.7e-03 &  5057 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   36.6 &  NaN \\
  9718066 &   16.1 &  142.5 &  K02287.01 &          planet &  1.0e-02 &  8.7e-04 &  4470 &    107 &   4.7 &  2.5e-02 &    0.6 &  3.3e-02 &   SM &    0.7 &  0.1 \\
  9729691 &    8.7 &  133.7 &  K01751.01 &          planet &  3.2e-02 &  1.4e-03 &  5165 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.7 &  NaN \\
  9735426 &    8.1 &  138.7 &  K01849.01 &          planet &  2.8e-02 &  5.9e-04 &  5170 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.2 &  NaN \\
  9758089 &   92.7 &  177.5 &  K01871.01 &  offset-no-star &  3.0e-02 &  1.5e-03 &  4569 &     48 &   4.7 &  1.3e-02 &    0.7 &  1.9e-02 &   SM &    2.1 &  0.1 \\
  9762519 &    7.5 &  138.1 &        NaN &          Vshape &  4.3e-01 &  4.3e-02 &  5709 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   42.1 &  NaN \\
  9765975 &   18.5 &  138.2 &  K01520.01 &          planet &  2.1e-02 &  6.4e-04 &  5372 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.9 &  NaN \\
  9783760 &   89.7 &  205.3 &        NaN &          Vshape &  2.9e-01 &  5.0e-02 &  5859 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   28.4 &  NaN \\
  9815053 &    5.8 &  136.9 &  K02923.01 &          planet &  1.5e-02 &  8.4e-04 &  5262 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.2 &  NaN \\
  9818462 &   25.9 &  156.2 &  K01521.01 &          planet &  2.2e-02 &  7.1e-04 &  5136 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.9 &  NaN \\
  9821078 &    8.4 &  132.3 &        NaN &         eclipse &  6.5e-01 &  1.1e-03 &  4246 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &   39.2 &  NaN \\
  9838468 &   54.4 &  175.4 &  K02943.01 &          planet &  1.3e-02 &  1.1e-03 &  5750 &     37 &   4.3 &  9.1e-02 &    1.2 &  1.5e-01 &   SM &    1.7 &  0.3 \\
  9846086 &   37.9 &  160.8 &  K00617.01 &          planet &  1.3e-01 &  4.8e-03 &  5781 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   12.7 &  NaN \\
  9849884 &    5.4 &  131.6 &        NaN &          planet &  7.8e-03 &  9.5e-04 &  6093 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    0.8 &  NaN \\
  9850893 &    8.5 &  135.8 &  K01523.01 &        vardepth &  1.6e-02 &  4.9e-04 &  5263 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.4 &  NaN \\
  9851271 &    8.5 &  135.9 &  K02003.01 &          planet &  1.8e-02 &  4.3e-04 &  5881 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.1 &  NaN \\
  9851662 &   15.1 &  135.5 &  K02483.01 &          planet &  1.4e-02 &  1.5e-03 &  5520 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.4 &  NaN \\
  9873254 &   14.7 &  131.7 &  K00717.01 &          planet &  1.5e-02 &  6.0e-04 &  5641 &     45 &   4.4 &  5.7e-02 &    1.1 &  7.8e-02 &   SM &    1.8 &  0.1 \\
  9886661 &    5.1 &  133.2 &  K01606.01 &          planet &  1.5e-02 &  5.3e-04 &  5403 &     43 &   4.5 &  3.9e-02 &    0.9 &  3.0e-02 &   SM &    1.5 &  0.1 \\
  9895006 &   10.6 &  133.8 &  K01717.01 &          planet &  1.5e-02 &  1.9e-03 &  5440 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.6 &  NaN \\
  9910828 &    8.5 &  135.9 &        NaN &          planet &  1.4e-02 &  9.2e-04 &  5504 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.3 &  NaN \\
  9941387 &   27.7 &  141.3 &        NaN &          radius &  7.6e-01 &  2.6e-02 &  5298 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   62.2 &  NaN \\
  9941859 &    9.6 &  138.4 &  K00528.01 &          planet &  2.7e-02 &  2.6e-03 &  5675 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    3.1 &  NaN \\
  9957627 &   39.8 &  135.7 &  K00592.01 &          planet &  2.1e-02 &  8.4e-04 &  6090 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.4 &  NaN \\
  9958962 &   10.0 &  131.8 &  K00593.01 &          planet &  2.3e-02 &  1.0e-03 &  5964 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.3 &  NaN \\
  9962455 &   23.2 &  142.6 &  K02748.01 &          planet &  1.5e-02 &  1.1e-03 &  5426 &    151 &   4.0 &  2.5e-01 &    1.9 &  6.2e-01 &   SM &    3.0 &  1.0 \\
  9962595 &   11.4 &  142.4 &        NaN &          planet &  1.5e-01 &  2.1e-03 &  5264 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   13.1 &  NaN \\
  9963009 &   40.1 &  153.0 &        NaN &         eclipse &  2.1e-01 &  2.2e-04 &  5795 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &   25.9 &  NaN \\
  9963524 &    5.7 &  134.2 &  K00720.01 &          planet &  3.3e-02 &  4.0e-04 &  5246 &     84 &   4.6 &  1.7e-02 &    0.8 &  2.9e-02 &   SM &    2.9 &  0.1 \\
  9964801 &   13.7 &  139.5 &  K00721.01 &          planet &  1.8e-02 &  1.9e-03 &  5819 &     54 &   4.3 &  6.0e-02 &    1.2 &  8.4e-02 &   SM &    2.3 &  0.3 \\
  9967884 &    5.4 &  131.8 &  K00425.01 &          planet &  1.4e-01 &  8.3e-03 &  5866 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   13.3 &  NaN \\
  9973109 &   27.5 &  133.3 &  K02018.01 &          planet &  2.2e-02 &  1.6e-03 &  5707 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.5 &  NaN \\
  9991621 &   18.9 &  145.5 &        NaN &        vardepth &  1.1e-02 &  5.0e-04 &  5456 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.1 &  NaN \\
  9993683 &   29.9 &  145.1 &        NaN &          planet &  1.5e-02 &  1.2e-03 &  5241 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.3 &  NaN \\
 10004738 &   56.5 &  143.8 &  K01598.01 &          planet &  3.2e-02 &  3.4e-03 &  5816 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.1 &  NaN \\
 10006581 &   40.1 &  142.1 &  K01595.01 &          planet &  2.6e-02 &  1.6e-03 &  5965 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.6 &  NaN \\
 10016874 &   16.3 &  139.5 &  K00426.01 &          planet &  2.7e-02 &  1.0e-03 &  6059 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    3.4 &  NaN \\
 10019643 &   21.3 &  150.4 &  K00471.01 &          planet &  2.4e-02 &  1.5e-03 &  5732 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &    2.3 &  NaN \\
 10022908 &    7.0 &  135.5 &  K01586.01 &          planet &  2.2e-02 &  1.3e-03 &  4735 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.5 &  NaN \\
 10024701 &   14.4 &  139.1 &  K02002.01 &          planet &  1.5e-02 &  1.0e-03 &  5935 &    109 &   4.4 &  4.0e-02 &    1.1 &  5.4e-02 &   SM &    1.7 &  0.1 \\
 10028792 &  114.7 &  165.1 &  K01574.01 &          planet &  6.6e-02 &  1.6e-03 &  5802 &     64 &   4.3 &  1.3e-01 &    1.3 &  2.4e-01 &   SM &    9.4 &  1.8 \\
 10031885 &    8.6 &  132.0 &  K00329.01 &         eclipse &  1.4e-02 &  2.2e-04 &  6035 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.4 &  NaN \\
 10031907 &    8.6 &  132.0 &        NaN &         eclipse &  2.8e-02 &  1.6e-04 &  5632 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.5 &  NaN \\
 10031918 &    8.6 &  132.0 &        NaN &          planet &  1.0e-02 &  7.9e-04 &  4944 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    0.8 &  NaN \\
 10033279 &   72.5 &  139.8 &  K01604.01 &          planet &  3.1e-02 &  1.7e-03 &  5812 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    3.6 &  NaN \\
 10053138 &   11.8 &  138.8 &        NaN &          planet &  8.9e-03 &  6.5e-04 &  5703 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &    0.8 &  NaN \\
 10063208 &    9.3 &  132.9 &        NaN &          planet &  5.6e-03 &  3.5e-04 &  5780 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    0.5 &  NaN \\
 10064256 &    6.0 &  135.0 &  K02849.01 &          planet &  1.0e-02 &  8.4e-04 &  5301 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    0.9 &  NaN \\
 10098844 &   47.4 &  173.5 &  K02964.01 &          planet &  1.8e-02 &  5.8e-04 &  6008 &    192 &   4.3 &  3.6e-02 &    1.1 &  4.3e-02 &   SM &    2.2 &  0.1 \\
 10122255 &   27.7 &  144.9 &  K01086.01 &          planet &  2.1e-02 &  1.0e-03 &  6057 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    2.4 &  NaN \\
 10134152 &   39.3 &  154.9 &  K02056.01 &          planet &  2.2e-02 &  1.4e-03 &  6060 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.3 &  NaN \\
 10136549 &    9.7 &  132.8 &  K01929.01 &          planet &  1.2e-02 &  7.9e-04 &  5681 &    184 &   4.1 &  2.7e-01 &    1.6 &  6.3e-01 &   SM &    2.0 &  0.8 \\
 10154388 &   12.1 &  138.2 &  K00991.01 &          planet &  1.8e-02 &  1.1e-03 &  5541 &     43 &   4.4 &  5.1e-02 &    0.9 &  5.0e-02 &   SM &    1.8 &  0.1 \\
 10155434 &   12.7 &  142.5 &  K00473.01 &          planet &  2.6e-02 &  1.3e-03 &  5541 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.3 &  NaN \\
 10158418 &    5.0 &  135.0 &  K01784.01 &          planet &  5.6e-02 &  2.0e-03 &  5956 &    108 &   4.4 &  4.2e-02 &    1.0 &  6.3e-02 &   SM &    6.3 &  0.4 \\
 10187159 &    8.0 &  136.8 &  K01870.01 &          planet &  2.6e-02 &  1.6e-03 &  5101 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
 10189542 &   24.6 &  142.5 &        NaN &          planet &  1.6e-02 &  2.4e-03 &  5645 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.5 &  NaN \\
 10189546 &   24.6 &  142.5 &  K00427.01 &  offset-no-star &  3.6e-02 &  1.2e-03 &  5462 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.4 &  NaN \\
 10190075 &   11.2 &  138.0 &  K03007.01 &          planet &  1.3e-02 &  1.5e-03 &  5879 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
 10198109 &   17.9 &  146.4 &        NaN &         eclipse &  3.2e-01 &  1.1e-04 &  5971 &    -99 &   4.0 &      NaN &    1.7 &      NaN &    P &   57.2 &  NaN \\
 10215422 &   24.8 &  154.1 &        NaN &         eclipse &  7.5e-01 &  1.4e-02 &  5615 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   68.6 &  NaN \\
 10252275 &   14.9 &  143.0 &  K03130.01 &          planet &  1.3e-02 &  1.1e-03 &  5141 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.1 &  NaN \\
 10266615 &   10.9 &  137.5 &  K00530.01 &          planet &  2.2e-02 &  1.6e-03 &  5720 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
 10268809 &   24.7 &  139.0 &        NaN &         eclipse &  2.5e-01 &  8.1e-03 &  6058 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   28.0 &  NaN \\
 10274244 &   13.7 &  135.2 &        NaN &         eclipse &  4.3e-01 &  1.0e-03 &  5453 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   39.2 &  NaN \\
 10285631 &   18.7 &  133.5 &  K00331.01 &          planet &  1.9e-02 &  1.1e-03 &  5689 &     44 &   4.4 &  4.9e-02 &    1.0 &  6.1e-02 &   SM &    2.1 &  0.2 \\
 10289119 &   16.1 &  135.0 &  K02390.01 &          planet &  1.0e-02 &  4.4e-04 &  6077 &     42 &   4.2 &  1.3e-01 &    1.4 &  2.6e-01 &   SM &    1.6 &  0.3 \\
 10290666 &    5.5 &  133.9 &  K00332.01 &          planet &  1.5e-02 &  8.8e-04 &  5720 &     43 &   4.2 &  1.2e-01 &    1.3 &  2.0e-01 &   SM &    2.2 &  0.3 \\
 10292238 &  143.1 &  245.5 &        NaN &          Vshape &  5.9e-01 &  7.1e-02 &  5687 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   54.4 &  NaN \\
 10319590 &   21.3 &  132.7 &        NaN &         eclipse &  2.0e-03 &  1.5e-03 &  5738 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    0.2 &  NaN \\
 10328393 &    7.6 &  136.0 &  K01905.01 &          planet &  1.7e-02 &  9.1e-04 &  4954 &     37 &   4.6 &  3.6e-03 &    0.7 &  1.8e-02 &   SM &    1.3 &  0.1 \\
 10330495 &   18.1 &  138.6 &        NaN &         eclipse &  2.2e-01 &  3.6e-04 &  5333 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   21.1 &  NaN \\
 10336951 &   38.2 &  166.0 &  K02401.01 &          planet &  2.3e-02 &  4.1e-03 &  4625 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.6 &  NaN \\
 10337517 &    7.1 &  136.4 &  K01165.01 &          planet &  2.1e-02 &  1.6e-03 &  5357 &     62 &   4.5 &  4.0e-02 &    0.9 &  4.1e-02 &   SM &    2.0 &  0.2 \\
 10345862 &   58.3 &  152.5 &        NaN &          radius &  2.2e-01 &  5.4e-04 &  5374 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &   21.6 &  NaN \\
 10353968 &    9.1 &  133.0 &  K00618.01 &          planet &  2.8e-02 &  4.4e-04 &  5591 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.6 &  NaN \\
 10384798 &   38.5 &  158.3 &  K01997.01 &          planet &  2.4e-02 &  1.1e-03 &  6019 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.4 &  NaN \\
 10404582 &   37.9 &  134.4 &  K02147.01 &          planet &  2.0e-02 &  2.1e-03 &  5867 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.0 &  NaN \\
 10420279 &   45.4 &  173.0 &        NaN &          Vshape &  8.6e-01 &  1.6e-02 &  5665 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   96.7 &  NaN \\
 10426656 &    6.1 &  135.9 &  K01161.01 &          planet &  1.9e-02 &  7.3e-04 &  5294 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    1.7 &  NaN \\
 10453588 &   68.9 &  160.3 &  K02484.01 &          planet &  1.1e-02 &  1.0e-03 &  5739 &    162 &   4.3 &  1.6e-02 &    1.1 &  3.6e-02 &   SM &    1.3 &  0.1 \\
 10480915 &   19.6 &  132.4 &  K02040.01 &          planet &  2.2e-02 &  2.7e-03 &  5623 &     88 &   4.4 &  5.8e-02 &    1.0 &  7.9e-02 &   SM &    2.4 &  0.4 \\
 10482160 &    7.3 &  137.3 &  K01170.01 &          planet &  2.3e-02 &  2.6e-03 &  5805 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.2 &  NaN \\
 10483644 &    5.1 &  133.3 &        NaN &         eclipse &  2.5e-01 &  5.2e-03 &  6056 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   25.6 &  NaN \\
 10490960 &    5.7 &  133.6 &        NaN &         eclipse &  6.7e-01 &  1.6e-03 &  5871 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &   85.4 &  NaN \\
 10513530 &   16.5 &  138.6 &  K00533.01 &          planet &  2.6e-02 &  1.6e-03 &  5335 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.5 &  NaN \\
 10514429 &   20.7 &  143.3 &        NaN &          planet &  1.1e-02 &  8.9e-04 &  5899 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &    1.4 &  NaN \\
 10514430 &   20.7 &  143.3 &  K00263.01 &          planet &  1.2e-02 &  7.6e-04 &  5903 &    130 &   4.4 &  3.1e-02 &    1.1 &  1.7e-02 &   SM &    1.4 &  0.1 \\
 10545066 &   19.8 &  138.2 &  K00337.01 &          planet &  1.9e-02 &  1.3e-03 &  5751 &     38 &   4.3 &  6.0e-02 &    1.1 &  9.1e-02 &   SM &    2.3 &  0.2 \\
 10554999 &    6.4 &  135.6 &  K00534.01 &          planet &  2.6e-02 &  1.5e-03 &  5283 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.1 &  NaN \\
 10577994 &    8.2 &  135.8 &  K00475.01 &          planet &  2.5e-02 &  4.3e-04 &  5236 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
 10586208 &   23.6 &  145.9 &  K01308.01 &          planet &  1.9e-02 &  4.1e-04 &  5647 &    157 &   4.2 &  2.9e-01 &    1.6 &  6.8e-01 &   SM &    3.3 &  1.4 \\
 10586744 &   21.4 &  143.6 &        NaN &          planet &  9.6e-03 &  6.2e-04 &  6035 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &    1.2 &  NaN \\
 10593626 &  289.9 &  133.7 &  K00087.01 &          planet &  2.2e-02 &  1.6e-03 &  5578 &     59 &   4.4 &  3.3e-02 &    0.9 &  3.0e-02 &   SM &    2.3 &  0.2 \\
 10599206 &   18.4 &  141.6 &  K00476.01 &          planet &  2.4e-02 &  1.1e-03 &  5139 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
 10600955 &   65.6 &  173.3 &  K02227.01 &          planet &  2.2e-02 &  2.6e-03 &  5819 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.4 &  NaN \\
 10616679 &    8.6 &  138.1 &  K00429.01 &          planet &  5.3e-02 &  9.2e-04 &  5254 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    4.8 &  NaN \\
 10656823 &    8.3 &  137.9 &  K00598.01 &          planet &  2.4e-02 &  1.1e-03 &  5292 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.0 &  NaN \\
 10657406 &   34.2 &  137.8 &  K01837.01 &          planet &  2.2e-02 &  8.2e-04 &  5166 &     46 &   4.6 &  3.3e-02 &    0.8 &  3.5e-02 &   SM &    1.9 &  0.1 \\
 10666242 &   87.2 &  153.4 &  K00198.01 &          Vshape &  1.8e-01 &  2.2e-02 &  5731 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &   16.5 &  NaN \\
 10674871 &   41.9 &  172.0 &        NaN &          planet &  3.0e-02 &  3.0e-03 &  5939 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.0 &  NaN \\
 10676014 &   16.8 &  139.8 &  K01797.01 &          planet &  2.8e-02 &  1.3e-03 &  4925 &     63 &   4.6 &  1.4e-02 &    0.7 &  2.3e-02 &   SM &    2.3 &  0.1 \\
 10709622 &   51.3 &  177.7 &  K02108.01 &          planet &  2.5e-02 &  1.7e-03 &  6096 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    3.1 &  NaN \\
 10717241 &   12.4 &  142.3 &  K00430.01 &          planet &  4.1e-02 &  5.7e-03 &  4286 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    2.5 &  NaN \\
 10724369 &   55.6 &  131.9 &  K01302.01 &          planet &  2.8e-02 &  3.3e-03 &  5906 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.8 &  NaN \\
 10753734 &   19.4 &  149.8 &        NaN &         eclipse &  6.6e-01 &  3.2e-03 &  5655 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   60.2 &  NaN \\
 10779233 &  201.1 &  187.6 &  K01989.01 &          planet &  2.5e-02 &  2.2e-03 &  5644 &     30 &   4.4 &  7.3e-02 &    1.0 &  9.1e-02 &   SM &    2.7 &  0.3 \\
 10793172 &   12.1 &  143.0 &  K02871.01 &          planet &  1.4e-02 &  1.6e-03 &  5678 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.2 &  NaN \\
 10794242 &    7.1 &  137.8 &        NaN &         eclipse &  4.2e-01 &  2.3e-04 &  5645 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   44.7 &  NaN \\
 10798331 &  147.3 &  148.8 &  K02373.01 &          planet &  2.1e-02 &  1.8e-03 &  5712 &     47 &   4.4 &  4.6e-02 &    1.1 &  6.6e-02 &   SM &    2.6 &  0.3 \\
 10798605 &   56.0 &  159.2 &        NaN &         eclipse &  3.4e-01 &  9.5e-03 &  5243 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &   29.9 &  NaN \\
 10798838 &   62.1 &  172.1 &        NaN &          radius &  2.8e-01 &  1.5e-02 &  5381 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &   26.9 &  NaN \\
 10810838 &   56.4 &  144.8 &  K00174.01 &          planet &  2.9e-02 &  1.9e-03 &  4752 &     69 &   4.6 &  1.3e-02 &    0.7 &  1.8e-02 &   SM &    2.2 &  0.2 \\
 10843590 &   18.9 &  141.0 &  K00431.01 &          planet &  3.1e-02 &  1.1e-03 &  5417 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    3.0 &  NaN \\
 10845188 &  249.4 &  279.6 &        NaN &          Vshape &  2.6e-01 &  2.4e-02 &  5982 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &   31.1 &  NaN \\
 10858832 &    5.3 &  132.2 &  K00432.01 &          planet &  3.1e-02 &  2.1e-03 &  6045 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    3.3 &  NaN \\
 10867062 &   34.3 &  143.5 &  K01303.01 &          planet &  2.4e-02 &  6.9e-04 &  5506 &    -99 &   4.1 &      NaN &    1.5 &      NaN &    P &    3.8 &  NaN \\
 10873260 &    5.9 &  136.1 &  K00535.01 &          planet &  3.1e-02 &  8.8e-04 &  6021 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    3.4 &  NaN \\
 10875245 &   14.7 &  138.8 &  K00117.01 &          planet &  2.2e-02 &  1.7e-03 &  5807 &     99 &   4.3 &  7.9e-02 &    1.3 &  1.2e-01 &   SM &    3.0 &  0.4 \\
 10878263 &    7.2 &  133.6 &        NaN &          planet &  2.6e-02 &  5.6e-04 &  5450 &     95 &   4.5 &  3.1e-02 &    0.9 &  3.2e-02 &   SM &    2.5 &  0.1 \\
 10880507 &    6.5 &  132.9 &  K02936.01 &          planet &  1.2e-02 &  1.5e-03 &  5690 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.1 &  NaN \\
 10908248 &   39.9 &  154.8 &  K03146.01 &          planet &  1.2e-02 &  7.8e-04 &  5902 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    1.4 &  NaN \\
 10917433 &    6.9 &  132.2 &        NaN &          planet &  5.4e-03 &  5.8e-04 &  5767 &    120 &   4.4 &  4.5e-02 &    1.1 &  5.7e-02 &   SM &    0.6 &  0.1 \\
 10917681 &   12.9 &  136.8 &        NaN &          planet &  1.9e-02 &  1.7e-03 &  6074 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.0 &  NaN \\
 10925104 &   11.8 &  142.7 &  K00156.03 &          planet &  3.3e-02 &  3.9e-04 &  4587 &     30 &   4.7 &  1.6e-02 &    0.7 &  2.1e-02 &   SM &    2.3 &  0.1 \\
 10933561 &   31.5 &  153.6 &  K00291.01 &          planet &  1.7e-02 &  3.2e-04 &  5727 &     38 &   4.3 &  1.1e-01 &    1.2 &  1.8e-01 &   SM &    2.3 &  0.3 \\
 10934674 &   16.5 &  136.6 &  K00477.01 &          planet &  2.5e-02 &  6.7e-04 &  5088 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.0 &  NaN \\
 10936427 &    7.2 &  131.7 &        NaN &         eclipse &  6.2e-01 &  5.0e-03 &  5333 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   51.5 &  NaN \\
 10964440 &   19.1 &  139.4 &  K01310.01 &          planet &  2.0e-02 &  1.3e-03 &  6045 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.1 &  NaN \\
 10965008 &   81.2 &  178.6 &        NaN &          planet &  3.2e-02 &  1.9e-03 &  5808 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    3.1 &  NaN \\
 10965963 &    6.6 &  132.8 &        NaN &         eclipse &  6.7e-01 &  1.5e-02 &  6056 &    -99 &   4.3 &      NaN &    1.2 &      NaN &    P &   87.0 &  NaN \\
 10973814 &   44.9 &  172.5 &  K01307.01 &          planet &  2.6e-02 &  1.2e-03 &  5783 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.9 &  NaN \\
 10977671 &  199.0 &  180.2 &        NaN &          planet &  1.4e-02 &  2.4e-03 &  5161 &    242 &   3.5 &  4.5e-01 &    3.4 &  1.5e+00 &   SM &    5.3 &  2.5 \\
 10990917 &   11.0 &  136.4 &  K01643.01 &          planet &  1.8e-02 &  1.3e-03 &  6072 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.0 &  NaN \\
 11015108 &   39.3 &  132.0 &  K00344.01 &          planet &  3.2e-02 &  1.4e-03 &  5581 &     59 &   4.4 &  3.6e-02 &    0.9 &  3.6e-02 &   SM &    3.2 &  0.2 \\
 11015323 &   34.2 &  159.2 &  K00479.01 &          planet &  3.0e-02 &  7.6e-04 &  5516 &     19 &   4.5 &  5.7e-02 &    0.9 &  5.1e-02 &   SM &    3.0 &  0.2 \\
 11017901 &    7.8 &  137.3 &  K01800.01 &          planet &  6.0e-02 &  3.5e-03 &  5540 &     93 &   4.5 &  2.7e-02 &    0.9 &  3.7e-02 &   SM &    5.8 &  0.4 \\
 11037335 &   40.7 &  146.6 &  K01435.01 &          planet &  2.2e-02 &  3.2e-04 &  5993 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.2 &  NaN \\
 11045383 &   41.2 &  158.9 &        NaN &          planet &  1.0e-01 &  1.2e-02 &  5199 &    -99 &   4.5 &      NaN &    0.8 &      NaN &    P &    9.0 &  NaN \\
 11069176 &   15.4 &  143.4 &  K02007.01 &          planet &  1.3e-02 &  1.2e-03 &  6063 &    -99 &   4.4 &      NaN &    1.1 &      NaN &    P &    1.4 &  NaN \\
 11075279 &  345.2 &  318.3 &  K01431.01 &          planet &  7.8e-02 &  1.6e-03 &  5494 &     74 &   4.4 &  6.3e-02 &    1.0 &  6.9e-02 &   SM &    8.6 &  0.6 \\
 11100383 &   12.9 &  132.0 &  K00346.01 &          planet &  2.9e-02 &  1.5e-03 &  5104 &     28 &   4.6 &  1.6e-02 &    0.8 &  1.7e-02 &   SM &    2.4 &  0.1 \\
 11124436 &   13.9 &  132.8 &        NaN &          planet &  1.1e-02 &  8.1e-04 &  5964 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.2 &  NaN \\
 11125797 &   12.3 &  143.7 &        NaN &          planet &  1.2e-02 &  1.1e-03 &  5444 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.0 &  NaN \\
 11147814 &   95.2 &  224.6 &        NaN &          Vshape &  4.3e-01 &  5.1e-02 &  4538 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &   28.2 &  NaN \\
 11153121 &   15.0 &  134.5 &  K01647.01 &          planet &  1.6e-02 &  6.5e-04 &  5741 &     50 &   4.4 &  2.4e-02 &    1.1 &  2.5e-02 &   SM &    1.9 &  0.1 \\
 11177543 &   38.3 &  142.1 &  K01648.01 &          planet &  1.8e-02 &  1.1e-03 &  5333 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.5 &  NaN \\
 11177676 &   47.0 &  175.4 &        NaN &          planet &  2.0e-02 &  7.1e-04 &  5586 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    1.8 &  NaN \\
 11192998 &    7.7 &  133.7 &  K00481.01 &          planet &  2.8e-02 &  6.3e-04 &  5429 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.4 &  NaN \\
 11193263 &    6.9 &  136.6 &  K01438.01 &          planet &  1.3e-02 &  5.7e-04 &  5767 &     32 &   4.2 &  6.7e-02 &    1.3 &  1.1e-01 &   SM &    1.9 &  0.2 \\
 11194032 &   28.5 &  158.9 &  K00348.01 &          planet &  3.8e-02 &  4.1e-04 &  4686 &     29 &   4.6 &  1.2e-02 &    0.7 &  1.6e-02 &   SM &    2.9 &  0.1 \\
 11250587 &    7.3 &  134.0 &  K00107.01 &          planet &  2.0e-02 &  6.8e-04 &  5883 &     81 &   4.3 &  7.3e-02 &    1.3 &  1.2e-01 &   SM &    2.8 &  0.3 \\
 11253711 &   17.8 &  149.2 &  K01972.01 &          planet &  1.9e-02 &  1.8e-03 &  6074 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.0 &  NaN \\
 11253827 &   88.5 &  182.7 &  K02672.01 &          planet &  5.6e-02 &  2.6e-03 &  5569 &     82 &   4.5 &  1.7e-02 &    0.9 &  3.2e-02 &   SM &    5.7 &  0.3 \\
 11255231 &   13.7 &  137.5 &  K03003.01 &     offset-star &  1.2e-02 &  8.4e-04 &  6058 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.3 &  NaN \\
 11288051 &   13.8 &  131.8 &  K00241.01 &          planet &  2.5e-02 &  9.3e-04 &  4987 &     24 &   4.6 &  8.7e-03 &    0.7 &  8.9e-03 &   SM &    1.9 &  0.1 \\
 11297236 &   88.6 &  145.5 &  K01857.01 &          planet &  2.4e-02 &  1.5e-03 &  5657 &     90 &   4.5 &  3.2e-02 &    0.9 &  3.7e-02 &   SM &    2.4 &  0.2 \\
 11305996 &   55.7 &  152.7 &        NaN &  offset-no-star &  2.0e-02 &  3.1e-03 &  4238 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.2 &  NaN \\
 11337833 &   51.3 &  153.5 &  K01651.01 &          planet &  2.3e-02 &  2.8e-03 &  6026 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.4 &  NaN \\
 11358389 &   10.7 &  132.0 &  K02163.01 &          planet &  1.5e-02 &  6.1e-04 &  5983 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.7 &  NaN \\
 11360805 &   26.8 &  140.7 &  K02422.01 &          planet &  1.9e-02 &  1.3e-03 &  5412 &    -99 &   4.4 &      NaN &    0.9 &      NaN &    P &    1.9 &  NaN \\
 11361646 &    8.0 &  134.7 &  K00330.01 &          planet &  1.9e-02 &  6.3e-04 &  5969 &    121 &   4.4 &  3.6e-02 &    1.1 &  3.5e-02 &   SM &    2.3 &  0.1 \\
 11391018 &   30.4 &  148.1 &  K00189.01 &          planet &  1.3e-01 &  9.0e-05 &  4905 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   10.0 &  NaN \\
 11392618 &  110.9 &  174.2 &        NaN &          planet &  2.0e-02 &  1.0e-03 &  5606 &    178 &   4.2 &  1.7e-01 &    1.4 &  2.5e-01 &   SM &    3.0 &  0.6 \\
 11394027 &   14.4 &  141.7 &  K00349.01 &          planet &  2.3e-02 &  1.3e-03 &  5725 &     50 &   4.4 &  4.5e-02 &    1.1 &  6.1e-02 &   SM &    2.9 &  0.2 \\
 11395587 &   13.0 &  138.3 &  K00350.01 &          planet &  1.9e-02 &  1.1e-03 &  5786 &     37 &   4.4 &  6.0e-02 &    1.0 &  7.1e-02 &   SM &    2.1 &  0.2 \\
 11402995 &   10.1 &  139.0 &  K00173.01 &          planet &  2.0e-02 &  3.4e-04 &  5707 &    141 &   4.3 &  1.6e-01 &    1.2 &  2.1e-01 &   SM &    2.5 &  0.4 \\
 11403389 &   45.1 &  133.6 &  K02482.01 &          planet &  1.9e-02 &  1.3e-03 &  5753 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &    1.8 &  NaN \\
 11413812 &    5.7 &  131.7 &  K01885.01 &          planet &  1.9e-02 &  1.3e-03 &  5973 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.9 &  NaN \\
 11415243 &  168.8 &  211.4 &        NaN &          planet &  2.3e-02 &  2.3e-03 &  4794 &     54 &   4.6 &  9.4e-03 &    0.7 &  4.4e-03 &   SM &    1.7 &  0.2 \\
 11449844 &   38.5 &  151.9 &  K00125.01 &          planet &  1.4e-01 &  6.8e-05 &  5486 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   12.9 &  NaN \\
 11450414 &   12.8 &  133.7 &  K01992.01 &          planet &  1.7e-02 &  6.6e-04 &  6069 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.8 &  NaN \\
 11461844 &   13.7 &  139.2 &  K02356.01 &          planet &  1.2e-02 &  6.7e-04 &  6055 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.2 &  NaN \\
 11462341 &   42.3 &  158.3 &  K02124.01 &          planet &  1.8e-02 &  8.3e-04 &  4252 &    -99 &   4.7 &      NaN &    0.6 &      NaN &    P &    1.1 &  NaN \\
 11495458 &   10.5 &  137.6 &  K02318.01 &          planet &  1.7e-02 &  1.3e-03 &  4702 &    -99 &   4.6 &      NaN &    0.6 &      NaN &    P &    1.2 &  NaN \\
 11498128 &  106.3 &  135.7 &  K02296.01 &          planet &  1.8e-02 &  1.4e-03 &  5673 &    103 &   4.4 &  3.9e-02 &    1.0 &  3.2e-02 &   SM &    1.9 &  0.2 \\
 11502172 &   25.4 &  135.6 &        NaN &         eclipse &  3.3e-01 &  1.1e-03 &  5787 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   34.1 &  NaN \\
 11506235 &   20.4 &  140.0 &        NaN &         eclipse &  3.0e-01 &  1.0e-03 &  5908 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   30.9 &  NaN \\
 11519226 &   22.2 &  148.5 &        NaN &         eclipse &  1.0e-01 &  2.4e-02 &  5938 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   10.4 &  NaN \\
 11521048 &   25.7 &  143.4 &  K00540.01 &        vardepth &  1.1e-01 &  5.0e-03 &  5569 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   10.9 &  NaN \\
 11521793 &   27.1 &  137.6 &  K00352.01 &          planet &  1.8e-02 &  6.3e-04 &  5855 &    176 &   4.3 &  1.6e-01 &    1.2 &  2.4e-01 &   SM &    2.4 &  0.5 \\
 11554435 &    9.4 &  140.1 &  K00063.01 &          planet &  5.9e-02 &  1.8e-03 &  5568 &     96 &   4.5 &  1.6e-02 &    0.9 &  2.9e-02 &   SM &    5.9 &  0.3 \\
 11601584 &   51.8 &  183.0 &  K01831.01 &          planet &  2.9e-02 &  1.1e-03 &  5192 &     39 &   4.5 &  2.5e-02 &    0.8 &  2.3e-02 &   SM &    2.7 &  0.1 \\
 11614617 &   24.8 &  142.1 &  K01990.01 &          planet &  2.0e-02 &  7.1e-04 &  6088 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    2.1 &  NaN \\
 11619964 &   10.4 &  132.7 &        NaN &         eclipse &  4.6e-01 &  1.4e-02 &  5899 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   50.4 &  NaN \\
 11623629 &   81.7 &  211.7 &  K00365.01 &          planet &  2.3e-02 &  9.0e-04 &  5613 &    238 &   4.4 &  1.6e-01 &    1.1 &  2.7e-01 &   SM &    2.7 &  0.7 \\
 11651712 &   14.5 &  140.5 &        NaN &          planet &  1.7e-02 &  1.2e-03 &  5996 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.7 &  NaN \\
 11656302 &   22.3 &  150.8 &  K00434.01 &         eclipse &  1.4e-01 &  4.8e-04 &  5700 &    -99 &   4.6 &      NaN &    0.9 &      NaN &    P &   12.6 &  NaN \\
 11656721 &   13.6 &  139.4 &  K00541.01 &          planet &  2.4e-02 &  1.0e-03 &  5536 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.1 &  NaN \\
 11656918 &   62.1 &  161.1 &  K01945.01 &          planet &  2.9e-02 &  2.1e-03 &  5434 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.5 &  NaN \\
 11657614 &    5.9 &  133.8 &        NaN &          planet &  1.5e-02 &  1.1e-03 &  4870 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.1 &  NaN \\
 11662184 &   27.6 &  145.4 &  K02791.01 &          planet &  1.7e-02 &  8.4e-04 &  6046 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.7 &  NaN \\
 11669239 &   41.9 &  136.8 &  K00542.01 &          planet &  2.5e-02 &  1.0e-03 &  5731 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.8 &  NaN \\
 11671579 &    5.2 &  133.8 &        NaN &          planet &  8.9e-03 &  7.6e-04 &  5557 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    0.8 &  NaN \\
 11702948 &    9.8 &  135.6 &  K01465.01 &          planet &  7.2e-02 &  4.7e-04 &  5811 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    6.9 &  NaN \\
 11709124 &   20.5 &  137.8 &  K00435.01 &          planet &  3.4e-02 &  7.0e-04 &  5706 &    101 &   4.4 &  6.3e-02 &    1.0 &  8.5e-02 &   SM &    3.7 &  0.3 \\
 11718144 &   16.5 &  134.0 &  K02310.01 &          planet &  2.0e-02 &  1.2e-03 &  5808 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.9 &  NaN \\
 11724210 &    5.7 &  132.0 &        NaN &         eclipse &  1.9e-01 &  2.0e-03 &  5971 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   21.5 &  NaN \\
 11754430 &   39.8 &  166.7 &        NaN &          planet &  1.5e-02 &  1.1e-03 &  5715 &    177 &   4.1 &  2.9e-01 &    1.8 &  7.8e-01 &   SM &    3.0 &  1.3 \\
 11760231 &   49.6 &  138.4 &  K01841.01 &          planet &  2.3e-02 &  9.0e-04 &  5151 &     41 &   4.6 &  3.1e-02 &    0.8 &  3.5e-02 &   SM &    2.0 &  0.1 \\
 11764462 &    5.7 &  136.6 &  K01531.01 &          planet &  1.2e-02 &  3.8e-04 &  5738 &    106 &   4.4 &  5.8e-02 &    1.0 &  8.0e-02 &   SM &    1.3 &  0.1 \\
 11769146 &  283.0 &  350.4 &        NaN &          Vshape &  6.8e-01 &  5.7e-02 &  5966 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   68.7 &  NaN \\
 11769689 &   14.7 &  135.6 &        NaN &          planet &  1.1e-02 &  7.1e-04 &  6078 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.2 &  NaN \\
 11769890 &  122.9 &  165.5 &  K01980.01 &          planet &  2.6e-02 &  3.5e-03 &  5413 &     42 &   4.5 &  3.1e-02 &    0.9 &  2.5e-02 &   SM &    2.6 &  0.3 \\
 11773022 &   45.2 &  159.1 &  K00620.01 &          planet &  7.1e-02 &  1.1e-04 &  6023 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    7.3 &  NaN \\
 11773328 &    8.7 &  134.6 &  K01906.01 &          planet &  2.8e-02 &  1.5e-03 &  5380 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &    2.4 &  NaN \\
 11774991 &   37.8 &  141.1 &  K02173.01 &          planet &  1.5e-02 &  5.4e-04 &  4705 &     52 &   4.6 &  5.3e-03 &    0.7 &  1.0e-02 &   SM &    1.1 &  0.0 \\
 11802615 &   28.9 &  149.6 &  K00296.01 &          planet &  2.2e-02 &  1.0e-03 &  5754 &     97 &   4.4 &  5.6e-02 &    1.0 &  7.7e-02 &   SM &    2.4 &  0.2 \\
 11812199 &   37.3 &  135.4 &        NaN &         eclipse &  1.1e-01 &  2.8e-03 &  5878 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &   10.5 &  NaN \\
 11818607 &    5.1 &  134.4 &  K02467.01 &          planet &  1.3e-02 &  1.4e-03 &  5885 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.3 &  NaN \\
 11818872 &   12.7 &  136.0 &  K02581.01 &          planet &  1.0e-02 &  8.9e-04 &  5424 &     38 &   4.5 &  2.4e-02 &    0.9 &  2.6e-02 &   SM &    1.0 &  0.1 \\
 11824222 &   15.8 &  145.5 &  K00437.01 &          radius &  2.1e-01 &  2.5e-02 &  5189 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   17.2 &  NaN \\
 11858541 &    5.7 &  135.7 &        NaN &         eclipse &  2.9e-01 &  2.2e-03 &  5585 &    -99 &   4.3 &      NaN &    1.1 &      NaN &    P &   34.0 &  NaN \\
 11869052 &   20.5 &  137.9 &  K00120.01 &             ttv &  1.5e-02 &  1.7e-03 &  5619 &    -99 &   4.2 &      NaN &    1.2 &      NaN &    P &    1.9 &  NaN \\
 11875734 &   99.7 &  208.4 &  K01828.01 &          planet &  3.4e-02 &  2.3e-03 &  5638 &    -99 &   4.2 &      NaN &    1.2 &      NaN &    P &    4.4 &  NaN \\
 11906217 &   37.9 &  162.5 &        NaN &         eclipse &  4.6e-01 &  1.7e-02 &  4772 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   33.0 &  NaN \\
 11909686 &  185.9 &  288.9 &        NaN &          planet &  1.0e-01 &  2.7e-02 &  5861 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    9.7 &  NaN \\
 11922778 &   65.4 &  176.3 &        NaN &          planet &  1.7e-02 &  1.7e-03 &  6010 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.8 &  NaN \\
 11955499 &    9.0 &  137.9 &  K01512.01 &  offset-no-star &  2.4e-02 &  6.8e-04 &  5118 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.9 &  NaN \\
 12055539 &   12.3 &  137.6 &        NaN &          planet &  1.4e-02 &  9.7e-04 &  6066 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.5 &  NaN \\
 12058204 &    5.5 &  132.8 &  K02218.01 &          planet &  1.5e-02 &  4.9e-04 &  5803 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.4 &  NaN \\
 12061222 &   17.2 &  140.6 &  K00484.01 &          planet &  3.0e-02 &  4.6e-04 &  5254 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    2.4 &  NaN \\
 12071037 &    6.1 &  135.1 &  K02388.01 &  offset-no-star &  9.8e-03 &  3.3e-04 &  5901 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.1 &  NaN \\
 12105785 &   32.0 &  142.7 &        NaN &         eclipse &  1.6e-01 &  2.1e-03 &  5508 &    -99 &   4.6 &      NaN &    0.8 &      NaN &    P &   13.8 &  NaN \\
 12106929 &    5.9 &  136.0 &  K00359.01 &          planet &  1.8e-02 &  3.8e-04 &  5954 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    1.8 &  NaN \\
 12107008 &    5.9 &  135.9 &        NaN &          planet &  9.9e-03 &  4.9e-04 &  5480 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    0.9 &  NaN \\
 12116489 &   25.3 &  137.4 &  K00547.01 &          planet &  4.4e-02 &  2.0e-03 &  5170 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    3.4 &  NaN \\
 12121570 &   91.5 &  165.7 &  K02290.01 &          planet &  2.5e-02 &  1.9e-03 &  4977 &     26 &   4.6 &  1.3e-02 &    0.7 &  1.7e-02 &   SM &    2.0 &  0.2 \\
 12154526 &   56.2 &  146.4 &  K02004.01 &          planet &  1.9e-02 &  2.0e-03 &  5663 &     63 &   4.3 &  1.4e-01 &    1.2 &  2.2e-01 &   SM &    2.5 &  0.5 \\
 12251650 &   17.8 &  138.7 &  K00621.01 &          planet &  2.0e-01 &  2.6e-02 &  5166 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   16.1 &  NaN \\
 12253474 &    6.4 &  135.6 &        NaN &          planet &  1.3e-02 &  5.8e-04 &  6085 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &    1.5 &  NaN \\
 12253769 &   20.6 &  141.1 &        NaN &  offset-no-star &  1.3e-02 &  9.0e-04 &  5450 &     63 &   4.5 &  2.7e-02 &    0.9 &  4.0e-02 &   SM &    1.3 &  0.1 \\
 12254792 &   40.4 &  139.5 &  K01506.01 &          planet &  2.8e-02 &  6.3e-04 &  5831 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.7 &  NaN \\
 12256520 &   33.2 &  143.4 &  K02264.01 &          planet &  1.7e-02 &  1.1e-03 &  5559 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    1.9 &  NaN \\
 12266636 &   33.4 &  148.9 &  K01522.01 &          planet &  2.2e-02 &  1.2e-03 &  5801 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &    2.4 &  NaN \\
 12301181 &    6.1 &  134.9 &  K02059.01 &          planet &  1.0e-02 &  4.7e-04 &  4999 &     59 &   4.6 &  1.2e-02 &    0.7 &  1.5e-02 &   SM &    0.8 &  0.0 \\
 12302530 &    5.9 &  133.3 &  K00438.01 &          planet &  3.2e-02 &  2.7e-03 &  4478 &     65 &   4.7 &  2.3e-02 &    0.6 &  3.4e-02 &   SM &    2.2 &  0.2 \\
 12306808 &   37.9 &  138.1 &        NaN &         eclipse &  6.6e-01 &  4.2e-03 &  6055 &    -99 &   4.5 &      NaN &    1.0 &      NaN &    P &   68.7 &  NaN \\
 12400538 &  150.2 &  138.3 &  K01503.01 &          planet &  5.1e-02 &  3.6e-03 &  5598 &     89 &   4.5 &  3.5e-02 &    1.0 &  3.5e-02 &   SM &    5.3 &  0.4 \\
 12403119 &   76.1 &  199.5 &  K01478.01 &          planet &  5.5e-02 &  1.1e-03 &  5551 &     66 &   4.5 &  6.4e-02 &    0.9 &  6.9e-02 &   SM &    5.6 &  0.4 \\
 12404305 &   22.2 &  147.3 &  K00486.01 &          planet &  2.7e-02 &  1.6e-03 &  5566 &    161 &   4.4 &  3.5e-02 &    1.0 &  6.3e-02 &   SM &    3.0 &  0.3 \\
 12417486 &  155.0 &  213.5 &  K00622.01 &          planet &  7.1e-02 &  1.3e-03 &  5005 &     83 &   3.5 &  2.1e-01 &    3.3 &  7.5e-01 &   SM &   25.3 &  5.8 \\
 12454461 &    7.5 &  136.4 &  K02463.01 &          planet &  8.0e-03 &  5.5e-04 &  6027 &     56 &   4.3 &  1.2e-01 &    1.3 &  2.2e-01 &   SM &    1.1 &  0.2 \\
 12505654 &    5.2 &  135.0 &  K02353.01 &          planet &  2.1e-02 &  2.0e-03 &  5182 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &    1.7 &  NaN \\
 12508335 &   42.9 &  155.2 &  K00215.01 &          planet &  1.5e-01 &  4.4e-03 &  5802 &    -99 &   4.4 &      NaN &    1.0 &      NaN &    P &   17.1 &  NaN \\
 12557713 &    7.2 &  132.5 &        NaN &         eclipse &  2.9e-01 &  2.6e-02 &  4873 &    -99 &   4.6 &      NaN &    0.7 &      NaN &    P &   21.9 &  NaN \\
 12644769 &   41.1 &  132.7 &        NaN &        vardepth &  3.4e-01 &  1.6e-03 &  4198 &    -99 &   4.7 &      NaN &    0.5 &      NaN &    P &   19.9 &  NaN \\
 12735740 &  282.5 &  363.1 &        NaN &          planet &  8.9e-02 &  1.0e-03 &  5576 &     56 &   4.4 &  3.7e-02 &    0.9 &  3.6e-02 &   SM &    9.0 &  0.4 \\
 12735830 &   31.8 &  134.6 &        NaN &          planet &  1.9e-02 &  2.8e-03 &  4712 &    -99 &   4.6 &      NaN &    0.6 &      NaN &    P &    1.3 &  NaN \\
 12834874 &    7.7 &  134.7 &  K00487.01 &          planet &  2.4e-02 &  6.1e-04 &  5666 &    -99 &   4.5 &      NaN &    0.9 &      NaN &    P &    2.3 &  NaN \\

